Bridging the Gap Between Theory and Practice on Insertion-Intensive Database

With the prevalence of online platforms, today, data is being generated and accessed by users at a very high rate. Besides, applications such as stock trading or high frequency trading require guaranteed low delays for performing an operation on a database. It is consequential to design databases that guarantee data insertion and query at a consistently high rate without introducing any long delay during insertion. In this paper, we propose Nested B-trees (NB-trees), an index that can achieve a consistently high insertion rate on large volumes of data, while providing asymptotically optimal query performance that is very efficient in practice. Nested B-trees support insertions at rates higher than LSM-trees, the state-of-the-art index for insertion-intensive workloads, while avoiding their long insertion delays and improving on their query performance. They approach the query performance of B-trees when complemented with Bloom filters. In our experiments, NB-trees had worst-case delays up to 1000 smaller than LevelDB, RocksDB and bLSM, commonly used LSM-tree data-stores, could perform queries more than 4 times faster than LevelDB and 1.5 times faster than bLSM and RocksDB, while also outperforming them in terms of average insertion rate.

==> Old/BloomFilters.tex <==
\section{Bloom Filters}\label{sec:bloom}
As discussed previously, bloom filters are probabilistic structures that can be used to enhance the expected cost of a query, but they do not provide a performance guarantee and they cannot be used for range queries.

To use Bloom filters, when inserting $N$ keys in an NB-tree, consider maintaining two different NB-trees at the same time. One, called $T$, which is the exact NB-tree data structure discussed so far and includes all the keys. We maintain an additional NB-tree, called the \textit{skeleton tree}, $\mathcal{T}_s$, which is a copy of $T$, but only contains its s-nodes, s-keys (and the s-key pointers). $\mathcal{T}_s$ is essentially a B-tree, with branching factor $f$, whose nodes non-leaf nodes have between $\frac{f-1}{2}$ to $f-1$ keys. The property of the skeleton tree $\mathcal{T}_s$, is that if we traverse down the tree searching for a key $q$, and in our traversal, we reach the $j$-th node of the $i$-th level of $\mathcal{T}_s$, then, we know that if $q$ is in $T_i$ (i.e., $i$-th level of $T$), then it, in fact, has to be in $T_i^j$ (i.e., the $j$-th s-node in the $i$-th level of $T$). 

Now we set a Bloom filter, $b_i^j$, for each s-node of $T$. Thus, $b_i^j$, with a certain probability, can tell use whether $T_i^j$ includes a key $q$ or not. Furthermore, bloom filters can only provide false positives, which means that if $b_i^j$ returns false, then it is certain that $q$ is not in $T_i^j$. To search for $q$, we start our search from the root of $\mathcal{T}_s$. We check if $b_0^0$ indicates that $T_0^0$ can include $q$ or not. If yes, then we search $T_0^0$. If $T_0^0$ does not include $q$, then, we move down one level in $\mathcal{T}_s$ according to the pointers. We continue traversing down $\mathcal{T}_s$, for each level $i$, checking whether $b_i^j$ returns true, and if it does, and if we've reached the $j$-th node of the level $i$, then we search $T_i^j$ for $q$. We continue this until we reach the leaf level of $\mathcal{T}_s$, from which we can find which leaf level s-node of $T$ we need to search. We keep pointers in each node in $\mathcal{T}_s$ to the corresponding s-node in $T$ to be able to make the link between the two.

Overall, in the worst-case, we will need to go through all the levels of $\mathcal{T}_s$ and for each of them search $T$, leading to the worst-case running time of $O(\log_B s\log_f N)$ which is the same as before, and without using bloom filters. However, most of the times, we will only need to the perform $O(\log_B s)$ once. In this case, if the skeleton tree, $\mathcal{T}_s$ fits in-memory (which is typically true, as for instance, in our experiments, for an index of size $110GB$ with $10^10$ keys, $\mathcal{T}_s$ is less than $1MB$), the cost will be $O(\log_B s)$ with high probability, which is a constant (and if it doesn't, the cost will be $O(\log_B s + \log_f N)$ which is $O(\log_f N)$). That is, with bloom filters, NB-trees can still maintain their logarithmic factor edge over LSM-trees. Here, we have assumed that $f<B$, which is typically true to obtain low insertion cost.

Note that if we consider LSM-trees with fractional cascading \cite{LHY+10} we can observe that the method discussed in this paper can be used to apply Bloom filters to that data structure. That is, fences in \cite{LHY+10} (that contain pointers to the next level tree in an LSM-tree) can be used to create an skeleton tree as discussed above. However, to keep the skeleton tree in memory, we will need $O(\frac{N}{B})$ space compared with $O(\frac{N}{s})$ of NB-trees. Using both fractional cascading and Bloom filter for LSM-trees has not been discussed before in the literature, and can be done to increase the query time of LSM-trees to that of NB-trees. It is worth mentioning that although this improves the query performance of LSM-trees, insertion delay of LSM-trees is still worse than NB-trees, making NB-trees a better choice for indexing and data storage.

%Finally, it can be easily verified that maintaining $\mathcal{T}_s$ does not affect the asymptotic time and space complexity of NB-tree operations. Furthermore, $\mathcal{T}_s$ is typically small, and thus, not only it does not have a significant effect on the space occupied by an NB-tree, but also it is possible, in some scenarios, to keep it in memory. For instance, in our experiments, for an index of size $110GB$ with $10^10$ keys, $\mathcal{T}_s$ is less than $1MB$.


==> Old/DiskHeadMainMemoryTradeOff.tex <==
\section{Trade Off between the Number of Disk Heads and Main Memory}\label{sec:opt:discHead}
%Note that in the analysis provided above (as well as the LSM-tree analysis in Section \ref{sec:relatedWork}), we assumed that we can merge two components of order of size $sf^i$ and $s f^{i+1}$ with only a constant number of seeks. For this to be possible, we need to be able to perform sequential reads of the two components and sequential writes of the resulting component at the same time, which is not possible if we only have one disk head (because if we have only one disk head, the head will need to move between the components, incurring non-constant number of seeks). 
With less than three disk heads, to avoid performing seeks as much as possible, we can read from one disk location and buffer some of the data in the main memory, and move the disk head to the location and write the data. If we have two disk heads, we can buffer less data in main memory, compared with one disk head. Thus, there is a trade-off between the number of disk heads and the amount of main memory used for buffering. Note that how much buffer should be used depending on whether two disk heads or one disk head is available become a typical constraint optimization problem, to minimize the insertion cost given a memory budget. It is not difficult to formulate the insertion time based on the buffer size and the number of disk heads available, however, the optimization problems do not have closed form solutions and, for the sake of space, we do not get into the details of these optimization problems. In practice, a buffer of size similar to the s-node size, can result in $O(f)$ seeks for each merge (by for instance buffering half of the parent s-node and half of each child, reading the parent s-node incurs constant number of seeks, and the $f$ child s-nodes $O(f)$ number of seeks), which does not increase the insertion time by much, as $f$ is typically much smaller than $s$.

\if 0

Thus, we will need to be able to perform 3 concurrent sequential page I/Os, which means we need to have at least three disk heads to achieve this. As a result, in our analysis for both LSM-trees and NB-trees, a constant amortized number of seeks is only possible if we have at least three disk heads for our disk operations. However, if this is not possible, during our merge process, we will need to buffer some of the data from each component in the main memory. 

\subsection{Using Two Disk Heads.} If we have two disk heads, we can perform two disk reads and writes concurrently. Thus, in our merge procedure, we will need to first use one of the disk heads to read one of the two components to be merged partially, then move the disk head to the other component to be read, read that sequentially and write the output with the second disk head. This will mean that we will need to reserve some space in main memory for our merge process, which results in less space available for the in-memory component of the tree.

Imagine that we can store $M$ elements in main memory. Then, we will need $s$ of it for the main memory component and $R$ of it as reserved space for each merge. Therefore, $M=s+R$. The cost of each merge (i.e. the number of page I/Os) will still be the same, but now the merge of the $i$-th level with the $(i+1)$-th level will have an extra $2\times \frac{sf^i}{R}$ seeks, because we have two extra seek for every $R$ elements of the $i$-th level, as after the $R$ elements that are in memory for the $i$-th level are merged, the disk head that is reading the $(i+1)$-th level needs to move to the $i$-th level, read the next $R$ elements and move back and continue reading the $(i+1)$-th level. Now, if the merge at most reaches the $i$-th level, then it will need to perform $O(\sum_{j=0}^{i}\frac{sf^j}{R})$ seeks (because all the levels up to the $i$-th level will be merged), which is $O(\frac{sf^i}{R})$. Thus, the total number of seeks will be 

$$
O(\sum_{i=0}^{log_f N} \frac{N}{(s-f)f^i}\frac{sf^i}{R})
$$

which is 

$$
O(\frac{N \times s}{(s-f)R}log_f N)
$$

This results in the amortized insertion time of 

$$
O(\frac{flog_f N}{B})\TSeqW + O(\frac{log_f N}{R})\TSeek)
$$

To use the notation provided in Section \ref{sec:NB:I:T}, this will be the same as 

$$
O(\frac{1}{\alpha\epsilon B^{1-\alpha\epsilon}}\log_B N)\TSeqW + O(\frac{1}{\alpha\epsilon R}\log_B N)\TSeek
$$


\subsection{Using One Disk Head.} Consider the case when only one disk head is available for merging two components. In this case, we will need to use the disk to read parts of the first component, then move it to the second component and read parts of the second component, merge them in memory and move the head to write the merge output. This means that we need to buffer both of the $i$-th and $(i+1)$-th component.

Similar to before, assume that we have reserved enough space to buffer $R$ element in the main memory. Let $R_u$ be the amount of buffer we allocate to the upper level of the tree joining the merge, an let $R_l$ be the size of the buffer for the lower level, ($R=R_u+R_l$). Therefore, every time, we will read $R_u$ elements from the $i$-th level in the merge, and read $R_l$ elements from the $(i+1)$-th level. After the in-memory merge, all the elements of either $R_l$ or $R_u$ (or both) will be completely merged. Thus, we will need to go to either the $i$-the level or $(i+1)$-th level and refill the buffer. In total, the number of page I/Os will be the same as the case of having more disc heads, but we need to perform $O(\frac{sf^i}{R_u})$ seeks for reading the $i$-th level, $O(\frac{sf^{i+1}}{R_l})$ seeks for reading the $(i+1)$-th and $O(\frac{sf^i}{R_u}) + O(\frac{sf^{i+1}}{R_l})$ seeks for writing the output (because at most for every read seek there will be a write seek). If the last level a merge reaches is the $i$-th level, the the total number of seeks in that merge will be 

$$
\sum_{j=0}^{i}O(\frac{sf^j}{R_u}+\frac{sf^{j+1}}{R_l})
$$

which is $O(sf^i(\frac{1}{R_u}+\frac{f}{R_l}))$. To minimize the number of seeks, we will need to minimize $\frac{1}{R_u}+\frac{f}{R_l}$. Using the fact that $R=R_u+R_l$ and treating $f$ and $R$ as constants, this becomes a standard calculus minimization problem. Solving the minimization problem, we will get $R_u=\frac{R}{\sqrt{f}+1}$. Substituting the values, we will obtain that the minimum value for $\frac{1}{R_u}+\frac{f}{R_l}$ is $\frac{(\sqrt{f}+1)^2}{R}$ which is $O(\frac{f}{R})$ Therefore, the total number of seeks, using the same procedure as before, will be

$$
O(\frac{N \times s\times f}{(s-f)R}\times \log_f N)
$$

This results in the amortized insertion time of 

$$
O(\frac{flog_f N}{B})\TSeqW + O(\frac{f}{R}log_f N)\TSeek
$$

Using the notation provided in Section \ref{sec:NB:I:T}, we can write 

$$
O(\frac{1}{\alpha\epsilon B^{1-\alpha\epsilon}}\log_B N)\TSeqW + O(\frac{B^{\alpha\epsilon}}{\alpha\epsilon R}\log_B N)\TSeek
$$

Finally, to observe the trade off between the number of disk heads and memory used, note that when having at least three disk heads, we do not need any reserved buffer space in memory (in fact, having more than three does not provide any significant additional benefit for the merge procedure) and the amortized number of seeks can be reduced to $O(1)$. Having two, disk heads, will mean a memory space $R$ will be needed to ensure at most $O(\frac{log_f N}{R})$ seeks and one disk heads can ensure $O(\frac{flog_f N}{R})$ seeks with a memory buffer of size $R$. In practice, an approach similar to Section \ref{sec:NB:param} can be taken to find the value of $R$ that minimizes the insertion cost (keep in mind that $M=s+R$).

\fi

==> Old/FurtherImprovements.tex <==
\section{Tiering}\label{sec:tiering}
With tiering merge policy, when a level is full, it is added to the next level without merging it with the level until the level becomes full and then the entire level is merged together and sent to the level after that. Tiering has better insertion performance while leveling provides faster query performance. See \cite{DI18} for more discussion.

The merge policies we discussed for NB-trees so far are similar to the leveling category for LSM-trees. However, tiering policies can be implemented with slight modification of what we have discussed so far, and we omit the details here. The major idea in adopting tiering policies in NB-trees is that when merging a node with its children, we append the data to the children, without reading the children (we will need to reserve enough space for a child that there is enough space when new keys are appended to the child).  Thus, each child will include a number of sorted runs that need to be searched when querying a key. The s-keys of an s-node can be kept separately from the r-keys or they can be merged with each sorted run (which increases the size of the NBTree and insertion cost, but reduces query cost). Further considerations need to be put regarding when an s-node needs to split or a new s-key needs to be added to it. 












==> Old/Intro.tex <==
%Note that the columns of the table are measured in terms of time, not cost. That is, NB-trees provide a theoretical (as well as empirical) advantage over the existing methods when the performance is measured in terms of time, not cost. Nevertheless, they still match (or improve upon, in the case of LSM-trees) the theoretical performance of other data structures (such as B-trees with Buffer) when the performance is measured in terms of cost.
%TODO: Prob. in the literature review. The focus of this paper is on insertion-intensive workloads. Specifically, we consider data structures with insertion cost $c\log n$ for $c$ less than one and query cost $c'\log n$ for $c'$ larger than one. %TODO: we want logarithmic query time and the optimal for insertion is at least logartithmic? check the trade-off papers. Check the range of values with proven trade-off

%We study the insertion and query performance of \textit{write-intensive} data structures (i.e., data structures designed for insertion-intensive workloads) in terms of insertion and query \textit{time} as opposed to the traditional \textit{cost} measure. The notion of \textit{cost} is used to refer to the number of disk I/Os performed for each data structure operation, while \textit{time} refers to the actual time taken for performing each disk I/O, and is divided into \textit{transfer time} and \textit{seek time}. Although \textit{transfer time} is proportional to I/O \textit{cost}, \textit{seek time} is not. Given the fact that, per page and on average, seek time can take 100 times longer than transfer time for hard disks \cite{S17} (see Section \ref{sec:term}), it is important to account for seek time in our analysis. 



\textbf{Insertion-intensive workload on large volumes.} Storage and access of the rapidly generated data on banking or trading systems \cite{M18}, social media \cite{F17a} or user logs \cite{I17, D17} have made providing fast read and write methods for accessing large datasets increasingly important. %TODO: Check the citations
Many such applications require databases that \textit{guarantee} high insertion rates while providing fast query performance. 



\textbf{The problem.} In database terms, the workload is insertion-intensive (i.e., operations performed are mostly insertions), the dataset is large and stored on secondary storage and the performance of a database system is measure by the following metrics: (1) \textit{worst-case insertion time} (2) \textit{worst-case query time} (3) \textit{amortized insertion time} and (4) \textit{expected query time}. There is in general a trade-off between optimizing insertion and query time and not all four metrics can be minimized at the same time. As our focus is on insertion-intensive workloads, we focus on designing data structures that primarily minimize insertion performance while forgoing query performance as little as possible. (3) and (4) affect the \textit{average} insertion or query rate a data structure can support over a set of keys inserted and queries, and allow for periods of low throughput (amortized and expected time are both \textit{average} in different sense of the word). A high worst-case insertion time can be unacceptable in many applications (such as the one mentioned above) and may result in data loss when data is inserted at a high rate in the database even if amortized insertion time is low. %TODO: Average query time? Bloom filters analysis

As we are considering storage on a secondary storage device (i.e., HDDs or SSDs), the insertion and query performance are dominated by disk read and writes. Accessing a page in secondary storage of size $B$ incurs two costs, one a \textit{seek} time and the other the \textit{sequential} read or write time. Seek time is the latency from the time the read or write request is sent to the disk until the time the data transfer starts and \textit{sequential} read or write time is the time taken to transfer the data. Sequential access time is typically determined by a devices bandwidth while seek time depends on internal mechanisms of the device, on HDDs it is the movement of the disk arm and platter, on SSDs it is the limitation of its electrical circuits. Sequential time is proportional to the size of the data transferred but seek time depends on how the data is stored, i.e., whether it is stored on contiguous blocks or not. It is important to account for seek time in our analysis as, per page, it can take multiple orders of magnitude longer than sequential access time (see Section \ref{sec:term} for more discussion). 

%Note that guaranteeing a low amortized time expected but a large worst-case time Since many existing databases are not able to guarantee a low worst-case insertion time, we also consider a more lenient requirement, that (3) the database needs to achieve a low \textit{amortized insertion time}. 

\textbf{LSM-trees.} In recent years, LSM-trees \cite{OCG+96, SR12, WXS+15, DFF17, LAK16, DI18, DI19} have attracted a lot of attention and are used as the de facto standard data structure for insertion-intensive workloads, such as in systems including levelDB\cite{G17}, BigTable \cite{CDG08}, HBase \cite{ABC+12}, RocksDB \cite{F17} (used by Google and Facebook \cite{CDG08, ABC+12, F17}), Cassandra \cite{LM10}, and Walnut \cite{CDM+12}. LSM-trees buffer insertions in an in-memory component and merge them down with on-disk components in bulk, creating sorted-runs on disk. They contain several on-disk components exponentially increasing in size, each kept as a B$^+$-tree. The in-memory component is of size $c$ and the $i$-th level on-disk component is of size $c\times f^i$ for parameters $c$ and $f$ (see Fig. \ref{fig:lsm-tree}). 

LSM-trees provide better insertion performance compared with B-trees for two reasons. One, their amortized insertion cost is lower than B-trees by the factor $\frac{f}{B}$, for page size $B$ ($f$ is typically orders of magnitude smaller than $B$). Secondly, they perform fewer seek operations than B-trees. B-trees perform at least one seek per insertion (as they update the secondary storage after every insertion) while LSM-trees perform constant number of seeks every $c$ insertions (as they buffer every $c$ insertion in memory and write them sequentially to disk, merging them with the on-disk component).

\textbf{LSM-tree Design Issues.} Although LSM-trees optimize amortized insertion time, their original design suffer from a suboptimal query time \cite{LHY+10} (higher than logarithmic in data size) and a high worst-case insertion time \cite{TY17} (linear in data size). By looking at their structure, we can trace these performance issues to the following flaws in their design.

\begin{itemize}
    \item \textbf{Disconnected Components}. No relationship is established between the keys stored in each component. As a result, queries between the levels have to search several B$^+$-tree components, resulting in a suboptimal query time \cite{LHY+10}.
    \item \textbf{Asymmetric Design.} Size of LSM-tree components grow exponentially across levels. Thus, Merge operations are more costly at the lower levels but occur less frequently. This asymmetry results in the unacceptable linear worst-case insertion cost \cite{TY17}.
\end{itemize}

\textbf{Existing Solutions.} Existing solutions have focused on improving LSM-trees' performance without alleviating the root cause of its performance bottlenecks that are inherent in its design.  Bloom filters (such as in \cite{SR12}), in practice, and fractional cascading (such as in \cite{LHY+10}), in theory, have been used to improve the query time for LSM-trees. However, Bloom filters do not enhance the suboptimal worst-case query time of LSM-trees. Fractional cascading solves the \textit{disconnected components} problem (thus providing asymptotically optimal query performance \cite{Y09}) but is incompatible with Bloom filters and provides a worse query performance in practice \cite{SR12} compared with Bloom filters that reduce the expected query cost but leave the worst-case suboptimal. 

In view of the mentioned design flaws, more recent works \cite{DI19, DI18, DAM+17, TY17} have focused on fine tuning LSM-trees' parameters and merge policies to optimized their performance. None of the improvements match the query performance of B-trees, while they suffer from large worst-case insertion time that affects the insertion throughput and causes long delays during insertions. 

%TODO: add more relavant citations based on the two problems in their desing

%Although there have been many improvements suggested for LSM-trees (such as avoiding rereading and rewriting the data at every level of the tree \cite{WXS+15, DFF17, LAK16} or fixing the number of components \cite{SR12}), 

%NB-trees retain all the benefits of LSM-trees and improve on their downfalls. Specifically, NB-trees can meet the three requirements mentioned earlier. NB-trees provide a query time that is a logarithmic factor smaller than LSM-trees and is asymptotically the same as B-trees. However, NB-trees (similar to LSM-trees) provide a significant improvement in the insertion time compared with B-trees by performing most of their disk page writes sequentially. They can achieve a worst-case insertion time logarithmic in the data size, much better than LSM-trees, and hence can sustain high insertion rates and avoid long insertion delays, as is often the case for LSM-trees during their merge process (as the worst-case insertion time for LSM-trees is linear in data size). Moreover, unlike fractional cascading, NB-trees can be complemented with Bloom filters to achieve a query time similar to B$^+$-trees in practice, without sacrificing their theoretical performance. 

%In our experiments, NB-trees could obtain an average insertion rate of more then 100,000 insertions per second, higher than levelDB\cite{G17}, on an index of size 110 GB and answer queries 4 times faster than levelDB\cite{G17}, a commonly used LSM-tree based data structure (such as in \cite{DAM+17, SR12, LAK16, WXS+15, SSM+13}). Moreover, NB-trees could perform insertions at rate 100,000 ins./s with almost no delay during the insertions, while LevelDB experienced delays of 7 hours in total for the same data size.
%TODO: Mention exp results

%Furthermore, we present a novel nested structure for storing and processing data in batches. We use the concept of \textit{structural trees} (s-tree), trees whose nodes, called \textit{structural nodes} (s-nodes), are also tree data structures. S-trees impose a tree structure on other tree data structures, that is, they manage the relationship and ordering of the data among these (smaller sized) tree structures. In this paper, we study the scenario when the s-tree is a B-tree and the s-nodes are B$^+$-trees. In this scenario, the data is stored in $O(\frac{n}{s})$ number of B$^+$-trees (where $n$ is the total number of elements and $s$ is the number of elements in each s-node), and how the data is spread among these s-nodes (i.e., the $O(\frac{n}{s})$ B$^+$-trees) to support fast and efficient insertions and queries is dictated by the s-tree, which, in this paper, constrains the s-nodes to follow a B-tree structure. 

==> Old/LSMTreeDiscussion.tex <==
\section{Discussion of LSM-Tree's Performance}\label{LSM:Detail}
Consider an LSM-tree with a multiplying factor $f$. In such a setting, the $i$-th component has size $C_i = C_1\times f^{i}$, where $C_1$ is the number of elements in the first component. Thus, the tree will have $O(\log_f N)$ number of components. As a result, the query cost in an LSM-tree is $O(\sum_{i=0}^{\log_f N}\log_B (C_1\times f^i))$ which is $O(\log_B f \times (\log_f N)^2)$, which can be rewritten as $O(\log_f B(\log_B N)^2$. Note that all the page reads here include a seek time. Hence, the worst-case query time is $O(\log_f B(\log_B N)^2)\times(\TSeek+\TSeqR)$

Furthermore, the amortized insertion cost can be shown to be $O(\frac{f}{B}\log_f N)$. To see this, note that the total cost of insertion is equal to the cost of merging the data between different components of the LSM-tree. When $N$ is the total number of elements inserted in the tree, the $i$-th component will be overfull and will be merged with its next component at most $\frac{N}{C_i}$ times. The cost of each merge for the $i$-th component will be $O(\frac{C_i + C_{i+1}}{B})$ because both the $i$-th and $(i+1)$-th component need to be read and merged. Thus, the merging of the $i$-th component incurs a total of $O(\frac{N}{C_i}\frac{C_i + C_{i+1}}{B})$ page I/Os and the total cost will be
$$
O(\sum_{i=1}^{\log_f N}\frac{N}{C_i}(\frac{C_i + C_{i+1}}{B}))
$$
which is equal to 
$$
O(\frac{N}{B}\sum_{i=1}^{\log_f N}\frac{C_{i+1}}{C_i})
$$
and 
$$
O(\frac{N}{B}\sum_{i=1}^{\log_f N}f) = O(\frac{N}{B}f\log_f N)
$$

Thus, the amortized cost of insertion of $N$ elements in an LSM-tree is $O(\frac{f}{B}\log_f N)$, which we can rewrite as $O(\frac{f\log_f B}{B}\log_B N)$. Note that for each merge only a constant number of page I/Os include seeks, as each component is read and written on the disk sequentially, assuming that there are 2 read heads and 1 write head available so that the disk head does not have to move between the components when reading and writing. Thus, the amortized number of seeks for insertion is $O(\sum_{i=1}^{\log_f N}\frac{1}{C_i})$ which is $O(\sum_{i=1}^{\log_f N}\frac{1}{C_1\times f^i})$ and is $O(\frac{1}{C_1})$ which is $O(1)$. Hence, we can write the amortized insertion time as $O(\frac{f\log_f B}{B}\log_B N)\TSeqW+O(1)\TSeek$. Thus, as can be seen, an LSM-tree performs a constant number of amortized seeks, but its number of page accesses compared with the B-tree data structures can be larger, depending on the parameter $f$. As a result, it's use is beneficial only if the potentially larger number of sequential I/Os does not offset the improved performance gained by lower number of seeks. This can be controlled by selecting a value of $f$ that balances the two depending on the difference between the cost of the seeks the and sequential I/Os (see \cite{OCG+96} for further discussion on parameters of LSM-tree). %TODO: Talk about the number of disk heads and NB-tree

In general, increasing the number of components improves the amortized insertion time but worsens the query time of an LSM-tree. The larger the number of components, the closer its performance becomes to an unordered log-structured data structure, and the smaller the number of components, the closer it becomes to a B-tree. It is worth mentioning that Implementations of LSM-tree that impose a maximum limit on the number of component for an LSM-tree independent of the data size (such as \cite{SR12} that uses 3 components) will adversely affect the insertion time as the size of the data grows. Because a large value of $f$ results in an excessively large number of sequential I/Os which would result in insertions taking longer. Thus, although a larger value for $f$ reduces the query time, it worsens the insertion time, in which case the LSM-tree looses its advantage on writing to B-tree with buffer. Various heuristics can be employed to avoid such a large number of I/Os (for instance in \cite{SR12}), but they do not provide a performance guarantee and might cause a large number of I/Os in the worst-case.


LSM-trees suffer from a large insertion delay because in the worst-case, all the data need to be rewritten if all the components are full. Because the components are written sequentially on the disk there is only one seek for each component, which result in an insertion delay of $O(\frac{N}{B})\TSeqW+O(\log_f B \log_B N)\TSeek$.

Moreover, for LSM-trees, there are methods (such as \cite{SR12, PYX17, ZXL+16}) to deamortize the insertion time and use background processes, in order to reduce the insertion delay. In such methods, a background process performs the merge operations for the on-disk components while the insertions in memory are happening. These methods do not provide any guarantee that the background processes finish the merge operations in time, and there is no theoretical result on how much they reduce the insertion delay, however, they can be useful in practice. Moreover, these methods typically increase the number of seek operations performed by an LSM-tree, and thus, can worsen the performance in terms of insertion time.  


==> Old/Memory.tex <==
\section{The use of the main memory}
So far we have mainly focused on the NB-tree structure and how it is stored on the disk. However, it is important to discuss how the data structure can use the main memory to enhance its performance. We first discuss what are the components that can be kept in main memory, and then show that the typical approach taken in LSM-trees \cite{DI18, DAM+17, SR12} is not valid when the size of the data is of the order of billions.  

There are a number of components of NB-trees that can be kept in main memory. 

For data insertion, as discussed previously, the root node will need to be kept in memory, which is of size $s$ and will require at most about $\frac{s}{B}$ pages (ignoring the size of the non-leaf levels of the tree). Note that we can always keep the pages of the \BPTree in each s-node full (except the last page) because we create each \BPTree from sorted data. Furthermore, depending on the number of disk heads available for merging (see Section \ref{sec:opt:discHead}), we might need a buffer of size $B_m$ pages during the merging process, in addition to a buffer for Bloom filters of size $\frac{s\times r}{8(B\times b)}$ pages of the nodes during the merge, in order to avoid seeks (where $r$ is the number of bits per entry in the bloom filter and $b$ is the size of an entry in bytes in the index). This means that we need a total of $s(\frac{1}{B} + \frac{r}{8Bb}) + B_m$ pages in memory for insertion. Note that the size of the Bloom filter is typically much smaller than the other two terms (typically, $r$ is  about 8 and $b$ is at least 16), and $B_m$ can be set to $\frac{s}{B}$ for the best insertion performance, which will result in a buffer of size about $\frac{2s}{B}$ pages.  

For better query performance, we would want to keep the non-leaf r-nodes of each s-node in memory, in addition to the Bloom filters for each s-node. At most, there are a total of about $\frac{2N}{s}$ s-nodes in an NB-tree, and for each s-node, there are about $\frac{s}{B^2}$ non-leaf nodes. Thus, for the best performance, we will need to keep $\frac{2N}{s}\frac{s}{B^2}+ \frac{N\times r}{8(B\times b)}$ which is $\frac{N}{B}(\frac{2}{B}+\frac{r}{8b})$ pages in memory. Similarly, for the analysis here, we have only considered the size of the leaf s-nodes, as they dominate the total size of the structure. 

Note that the same analysis holds for LSM-trees as well. For instance, for LevelDB, $s$ will be equal to the number of elements in each SSTable. 

\subsection{A Quantitative Analysis}
Consider the following setting to see in what circumstances caching this amount of metadata in memory is feasible. We follow our experimental setting in Section \ref{sec:exp}, for a machine with 4 KB pages and 4GB of main memory. For an index entry of size $b = 16$ and page size $B\times b = 4096$ we have that $B = 256$. Moreover, consider the case when the Bloom filters have 8 bits per element (i.e., $r = 8$).  Therefore, the total memory usage will be $\frac{N}{256}(\frac{2}{256}+\frac{1}{16}) + \frac{2s}{256}$ pages. Consider a main memory of size 4GB (which can fit $2^20$ pages).

Even assuming the $s$ is negligible compared with the other terms, we have that $N$ is at most $3.82\times 10^9$ (the actual value is in fact smaller because we have ignored some of the terms in the actual cost). This means that caching this amount of data in main memory is not possible when the number of items in an index are in the order of billions. In such a scenario, when the data size of of the order of billion elements, the analysis of \cite{DI18, DAM+17, SR12} which assumes that the bloom filters and the non-leaf level of the trees can fit in main memory does not hold.

\subsection{Buffering Priorities}
As discussed above, the main memory cannot be used to keep all the metadata for data of large size. Therefore, we need to decide how we allocate the memory between different components. For insertions, Section \ref{sec:opt:discHead} discusses the trade-offs between size of an s-node and the buffer used for merging.

For querying, we can keep the Bloom filters, as well as the non-leaf r-node of each s-node in main memory. If they all do not fit in main memory, we need to prioritize which ones are more important to be kept in main memory. One can formulate the problem of how much buffer should be allocated to Bloom filters and how much to caching the index given a memory space availability as a constrained optimization problem, minimizing the expected query cost subject to the memory constraint. For the sake of space, we leave out the technical details. In general, to decide how much of the main memory space should be allocated to Bloom filters and how much to caching the index, a main factor is the probability of a Bloom filter of an s-node returning negative regarding the existence of a queried element in the s-node. If this probability is high, the use of Bloom filters will be advantages, and if it isn't, Bloom filters will be redundant because the s-node needs to be checked very often. This probability depends on a number of factor such as the proportion of zero-result queries in the workload, the probability that a certain element in the NB-tree exists in a certain s-node when the s-node is queried and the false positive probability of the Bloom filter.  

\if 0

Let $s_b$ be the size of a Bloom filter for an s-node in pages. For an s-node, imagine that the proportion of a Bloom filter kept on disk compared with the proportion kept in memory is $p_r$. Assuming queries and the output of Bloom filter's hash functions are uniformly distributed, the expected number of disk accesses for such a Bloom filter for a query will be $p_r\times s_b$. 

Note that for a \BPTree in each s-node of height $h$, keeping the first $h-2$ levels in memory requires about $\frac{s}{B^3}$ pages (Which is about )

Note that a query, searches one s-node per level, during which it first checks the Bloom filter of the s-node, and depending on the result given by the Bloom filter, it may query the \BPTree in the node. If the Bloom filter is not kept in memory, and the Bloom filter uses $k$ hash functions, checking the Bloom filter incurs extra $k$ seeks. On the other hand, if the non-leaf levels of the \BPTree are not kept in memory, querying the s-node will need $\log_\frac{B}{2} s$ seeks. 

 because the Bloom filter for an s-node is about $\frac{rB}{8b}$ times larger than the non-leaf nodes of the \BPTree index (which is about 8 in our example above). This is while it can at most improve the performance with a certain probability by $\log_\frac{B}{2} s$ for the s-node (which is usually at most 5). 



Firstly, the probability of a queried element existing in an s-node. This probability depends on two component, first, the probability of the queried element existing in the entire data structure (i.e. what proportion of queries return a result and are not zero-result queries) and second, the probability of an element existing in the data structure being in a specific s-node. Let the probability of a query being a zero-result query be $p_z$. Moreover, let the probability of a non-zero-result query being in an s-node be $p_i$, when the query reaches the  $i$-th level of the NB-tree. Therefore, the probability of a queried element existing in a certain s-node is $(1-p_z)p_i^j$. This is the probability of a true positive for a Bloom filter. Secondly, there is a probability of false positive depending on a Bloom filters setting. Let that be $p_f$ be this probability. Therefore, the probability of a Bloom filter returning true is $(1-p_z)p_i^j + p_f$.

If this probability is low, the use of Bloom filters can have a significant improvement on the query time and we must consider using the cache for the Bloom filter, or even storing it on the disk and performing seeks

Therefore, the expected cost of querying an s-node is $((1-p_z)p_i^j + p_f)(C+R) + (1-(1-p_z)p_i^j - p_f)R$. 

The use of Bloom filters is advantages when m

Here we need to consider two types of queries, zero result queries (where the key queried does not exist in the data structure) and non-zero result queries (where the key queried does not exist in the data structure).

When the key exists in the data structure, first note that having a bloom filter for the last level of the tree is redundant. This is because if the key exists in the tree and a query reaches the last level of the tree, the key has to exist in the last level (or the query would have found it in the other levels first). Therefore, if most of the queries performed on a data structure correspond to keys that exist in the data structure, then we don't need to keep Bloom filters for the last level of the tree. As a result, this will reduce the size required by the Boom filters by a factor of $\frac{f}{2}$ (because there are at least a factor of $\frac{f}{2}$ fewer number of nodes in the second last level of the tree). 


A Bloom filter for an s-node will take $\frac{sr}{8Bb}$ pages will the non-leaf levels of a \BPTree will need $\frac{s}{B^2}$ pages. Therefore, the ratio between their size is $\frac{rB}{8b}$.   

\fi

==> Old/Merging.tex <==
\section{Implementation of  Insertions} \label{sec:merge}
So far we have provided a conceptual discussion on the insertion operation in an NB-tree. However, implementation of this operation to minimize insertion time when the data is stored on disk requires more discussion. We call operations that discuss how keys are moved between disk pages during an insertion \textit{merge and split operations}, or only merge operations for short. Here, we describe two merge operations, M\&S (for merge and split) and BM\&S (for background merge and split). M\&S has a constant factor better amortized insertion time and query time but BM\&S deamortizes the insertion operation and has a worst-case insertion time only logarithmic in the data size (an improvement over the linear worst-case guarantee of an LSM-trees and M\&S). Note that the merge operations discussed here are similar to \textit{leveling} merge policies in LSM-trees (see \cite{DI18} for more discussion) but  \textit{tiering} policies can also be used with NB-trees. 


The overall procedure of the merge operations discussed in this section is as follows. The insertion of a key $K$ into an NB-tree $T$ with root $T_0^0$ follows the steps shown below.

\begin{itemize}
	\item{Insert $K$ in B$^+$-tree $T_0^0$. Stop here if it has at most $s$ keys.}
	\item{Call a merge operation on $T_0^0$. If it returns any keys, insert them into $T_0^0$ as s-keys.}
\end{itemize}

Note that since $T_0^0$ is kept in memory, the first step is an in-memory insertion in an in-memory B$^+$-tree, and is done based on the description in Section \ref{sec:design:insertion}, and we do not discuss this step here. Next, we will discuss the second step shown above, by providing two different merge operations, M\&S and BM\&S.


\subsection{M\&S Operation (Merging and Splitting)}\label{sec:merge:merge}
The M\&S operation happens between parent s-nodes and their children. For efficiency purposes and to minimize the number of seeks, every M\&S function call operates on all sibling s-nodes of an overfull s-node, called parent s-nodes, and the child s-nodes for each overfull parent involved in the operation. Let the parent s-nodes be $P_1$ to $P_q$ for an integer $q$, $q \leq f$, and the child s-nodes of $P_i$ be $C_i^1$ up to $C_i^{k}$ for an integer $k$, $k \leq f$ and $1\leq i\leq q$. To minimize the number of seeks performed when calling M\&S, we ensure that the following properties hold for an NB-tree. 

\begin{itemize}
    \item \textit{sibling sequentiality.} All the s-nodes in the NB-tree (except the root that is in main memory) are written on disk  \textit{sequentially with their siblings} (i.e., they are written next to their siblings), in the increasing order of their smallest keys.
    \item \textit{d-node sequentiality.} For every s-node, all the d-nodes in a d-tree are written on disk sequentially and a leaf d-node with smaller keys is written before all the leaf d-node with larger keys (the leaf d-nodes can be separated by non-leaf d-nodes).
\end{itemize}

As a result of the above properties, during M\&S, a sequential scan from the beginning of $P_i$'s first child s-node's fist leaf d-node until the end of $P_i$'s last child s-node's last leaf d-node can retrieve all the keys in $C_i^1$ to $C_i^k$ sorted in ascending order. It also implies that a sequential scan of $P_i$ from its first leaf d-node to the last leaf d-node can provide all the keys from $P_i$ in sorted order. 

M\&S works as follows, when called on parent s-nodes $P_1$ to $P_q$. Let $\mathcal{N}$ be the set of oversized s-nodes among $P_1$ to $P_q$. 

\begin{itemize}
	\item{If $P_1$ to $P_q$ are not leaf s-nodes, for every $P_i\in\mathcal{N}$,}
	\begin{itemize}
		\item{\textit{Merge Down Step.} Move r-keys of $P_i$ to its children}
		\item{\textit{Recursive Step.} Recursively call M\&S on $P_i$'s children if any of them becomes oversized}
	\end{itemize}
	\item{\textit{Update and Split Step.} For every $P_i\in\mathcal{N}$, if $P_i$ is a leaf s-node, split it and add the median key of $P_i$ to a set $M$. Otherwise,}
	\begin{itemize}
	    \item Update leaf d-node pointers, $P_{s-node}$, in s-node $P_i$. 
	    \item Update pointers associated with s-key of s-node $P_i$. 
	    \item If the recursive M\&S call on the children of $P_i$ has returned any s-keys, insert them in $P_i$.
	    \item If $P_i$ has more than $f-1$ s-keys, split it into two. Add the median s-key of $P_i$ to a set $M$.
	\end{itemize}
    \item{return $M$.}
\end{itemize}

%The M\&S operation is a recursive algorithm. Its base case is when the input s-nodes are leaf s-nodes, when the algorithm only splits the oversized s-nodes into two. Otherwise, it merges down the r-keys and recursively calls M\&S operation on any oversized children created. If the recursive calls of M\&S results in any splits and any s-keys need to be inserted in the s-node, the algorithm inserts them into the s-node and updates all of the s-nodes pointers.

More specifically, the merge down step performs Case (1) and Case (3) step in our insertion discussion (in Section \ref{sec:design:insertion}), but removing the r-keys from the parent s-node and updating the pointers in the parent s-node are postponed to the update and split step.  This step performs the insertion of the r-keys from a parent s-node to its children s-nodes and it does it in bulk and sequentially. That is, it scans a parent node $P_i$, $P_i\in\mathcal{N}$ and all it's children sequentially from their first leaf d-node to their last leaf d-node (ignoring non-leaf d-nodes if encountered). Because of the sequentiality properties above, this allows us to read all the r-keys in a sorted order in the parent and child s-nodes. Because the data is retrieved in a sorted order, we can construct a B$^+$-tree from it by only sequential writes (using a bulk loading approach similar to the LSM-tree merge operation). Since all the children resulting from a merge are written together, and because the B$^+$-tree in each child is created sequentially and written to the disk based on the sorted order of the keys, the resulting s-nodes preserve both of the sequentiality properties. Note that setting the pointers in the newly constructed s-nodes is done during the sequential construction of the B$^+$-tree of the s-node, and based on the rules discussed in Section \ref{sec:design:insertion}.

After the merge down step and the recursive calls, the update and split step performs the remainder of the insertion operation discussed in Case (1) and Case (3) as well Case (2) in Section \ref{sec:design:insertion}. That is, it removes the r-keys (that were moved down) from the parent s-node and updates all the d-node pointers, $P_{s-node}$, of all leaf d-nodes in $P_i$ as well as pointers associated with s-key of the s-node $P_i$. Moreover, in case the recursive step of the M\&S returns a non-empty set of s-keys, the s-keys are inserted into $P_i$ based on the discussion in Case 2 of Section \ref{sec:design:insertion}. Furthermore, if the s-node is a leaf s-node and it is oversized, or, if it is a non-leaf s-node and it has more than $f-1$ s-key, it splits the s-node into two and returns the median key. However, the update and split step, does all this in one sequential scan of all the sibling s-nodes $P_1$ to $P_q$. That is, it scans all the siblings sequentially. If it isn't oversize, it just writes it back to the disk in a new location. But if it is oversized, it performs all the discussed steps during the sequential scan. Note that all the steps in the update and split step can be done during sequentially writing $P_i$ and all the updates to $P_i$ are done based on the rules discussed in Section \ref{sec:design:insertion}. Moreover, this step also preserves the sibling and d-node sequentiality properties, because all sibling s-nodes $P_1$ to $P_q$ are written to the disk sequentially next to each other.

Here, we assume that $s < \frac{M}{3}$, such that we can store in memory during a merge $s$ of the parent s-node and $s$ keys for the output buffer (in addition to the root s-node). This way, we first read the parent s-node, buffer it in memory and sequentially read the child s-nodes until there are $s$ keys in the output buffer, then write the output buffer and move back to continue reading the child s-nodes. Note that having more hard disks can reduce this memory requirement as it will allow us to read and write from the hard disks simultaneously. 

\if 0


\subsubsection{Flushing down Step.} This step is done very similarly to the LSM-trees' merge procedure and thus we will only discuss the differences between the two here. We start the flushing down step by performing the merge of $P_i$ and $C_i^1$ into ${C_i^1}'$ using the same procedure as the LSM-tree merge (see \cite{OCG+96} for details). However, we need to discuss our treatment of s-keys which do not exist in LSM-trees and the fact that $P_i$ has several children. When we encounter an s-key in $P_i$, we do not write it to the output B$^+$-tree. Assume that we are merging $C_i^j$ and $P_i$ when we reach an s-key, $K$, in $P_i$ (s-keys in $C_i^j$ are written to the output just like its r-keys). This means that, all the keys in $C_i^j$ are written to the output B$^+$-tree ${C_i^j}'$ (this is because of the NB-tree cross-s-node linkage property discussed in \ref{sec:NBTreeDesign} that all the keys in $C_i^j$ are smaller than $K$). Hence, ${C_i^j}'$ is now complete and writing it has been finished. We move on to merging $P_i$ with $C_i^{j+1}$ into ${C_i^{j+1}}'$, reading the keys of $P_i$ from the next key after $K$. 

It is easy to see that this step preserves the sibling sequentiality of the tree, as the s-nodes are written in order and right after each other. Moreover, a typical bulk loading algorithm for B$^+$-tree can be utilized to write each s-node (as the data is read and written in a sorted order), which obviously preserves the d-leaf sequentiality. 

In Figure \insFigNo, this step has been applied to the root s-node in \insFigNo (c) to flush down 10, 29, 49, ..., 98 from the root s-node to its children. The result of the step can be seen in Fig. \insFigNo (d), where the elements are moved dowon the the leaf level s-nodes from the root s-node.

\subsubsection{Recursive Step.} After flushing down the keys, the size of the newly created children ${C_i^1}'$ to ${C_i^k}'$ is increased. As a result, we need to check whether they meet the size requirement or not, i.e. their size is at most $s$ (their number of s-keys has not changed). If all the $k$ children meet the size requirement, we will skip this step.

Otherwise, if there exits a child that is overfull, we recursively call M\&S on the children (the M\&S call is on all the children, because they are siblings). Note that such a recursive call might result in a child, ${C_i^j}'$ being split, which means we will need to insert a new s-key $K$ into $P_i$. %Let the set $E_s^i$ include the s-keys that need to be inserted into $P_i$ (the set will be returned by the merge function call). Furthermore, let the set $R_i$ be the set of root d-node of the B$^+$-tree in $R_i_j$ for each child $C_i^j'$ after the recursive merge call (this will also be). 

\subsubsection{Update and Split Step.} First note that to preserve sibling sequentiality, we will need to keep all the sibling s-nodes $P_j$ written next to each other. This is while $P_i$ for some $i$ values were not oversized and have not been modified at all. As a result, to preserve sibling sequentiality, we copy and rewrite $P_i$ for these $i$ values, without modification. Thus, in this step, we read all the $P_i$ s-nodes for all $i$ between 1 to $q$ and write them in order, while only modifying s-nodes that were oversized before the M\&S call.

For values of $i$ for which $P_i$ was oversized, We need to perform several operations. Let $P_i'$ be the s-node to be written instead of $P_i$ at this step. There are two cases depending on whether $P_i$ is a leaf s-node or not. 

\paragraph{Leaf s-nodes} Leaf s-nodes have no children and thus no pointers to be updated. Thus, here, we only need to split them if their size is larger than $s$ (note that the flushing down step was not performed for the leaf s-nodes). Similar to the splitting case for the non-leaf s-nodes, we can also easily split the node into two during our linear scan. However, this time, instead of adding the median of s-keys to $K_m$, we add the median of the r-keys to $K_m$ (note that all the keys in a leaf s-node are r-keys). Similarly, we 
return $K_m$ as the output of the M\&S function. As an example, the insertion of the key 8 in Fig. \insFigNo (e) and the flushing down step, results in splitting of the second leaf s-node. The split results in moving up the key 49 to the parent s-node, as shown in Fig. \insFigNo (f).

\paragraph{Non-leaf s-nodes.} First, note that up to this step of the algorithm, we have not yet removed the r-keys from $P_i$. This is done here, by discarding all the r-keys of $P_i$ and not writing them to $P_i'$. Secondly, the flushing down step has definitely changed the location of all of $P_i$'s children, to which $P_i$ keeps a pointer (and their location might have changed again during the recursive call step). Thus, the $P_i$'s pointers need to be changed. We do not get into the tedious details, but it can easily be seen that a linear scan of $P_i$ and writing it to $P_i$' can take care of all the pointer modifications. 

Finally, the recursive calls might have resulted in the split of some of $P_i$'s children, which means that new s-keys might need to be written in $P_i'$. Let $K^i$ be the set of s-keys needed to be written in $P_i'$. Writing these new keys in $P_i'$ can also be done easily during the linear scan of $P_i$. However, we need to make sure the number of s-keys in $P_i$' does not become more than $f-1$. If it does, while writing $P_i'$ we need to split it into two. Because we are writing the keys in an ascending order, the split can also be easily done. We count the number of s-keys written and when reaching the median instead of writing it we store it in a set $K_m$, and move on to writing a new s-node. Since we do this for all the values of $i$ that such that $P_i$ was oversized before the M\&S call, $K_m$ can contain more than one s-keys after writing all the s-nodes. We will return the set $K_m$ from the M\&S function as the output of the function call.

As an example, the insertion of the key 12 in Fig. \insFigNo (g) and the resulting flush down step, recursive calls and leaf s-node splits, results in the s-key 15 to be inserted in the non-leaf s-node, whose number of s-keys becomes more than 2, surpassing the limit, and resulting in the split of the root s-node into two. The root s-node is then split into two and a new root s-node is created, increasing the height of the tree by one. The result is shown in Fig. \insFigNo (h).

It is easy to see that this step also maintains the sequentiality properties of an NB-tree.

\fi


%\subsubsection{Insertion Time Complexity}\label{sec:NB:I:T}

\begin{theorem}[Time Complexity]\label{thm:timeInsertion}
The amortized insertion time of insertions using M\&S is $O(\log_f(\frac{N}{s})\times (\frac{f}{B}\TSeqW + \frac{f}{s}\TSeek))$.
\end{theorem}

\textit{Proof Sketch.} There are at most $O(\frac{N}{s})$ merges between any two level and each merge requires $O(\frac{fs}{B})$ page accesses, and the height of the s-tree is $O(\log_f \frac{N}{s})$. Assuming $s < \frac{M}{3}$, each merge can be handled with at most $O(f)$ seeks. 

\hfill\ensuremath{\square} 


\subsection{BM\&S (Background Merging and Splitting)}
Next, BM\&S, achieves a worst-case insertion time that is logarithmic in data size, allowing for low insertion delay. 

To present BM\&S we make the following modification in our assumptions. For non-leaf s-nodes, we remove the requirement on the maximum size of an s-node being $s$, and instead put a requirement on the total number of r-keys in all sibling s-nodes to be $f(s-f)$ (each s-node can still have at most $f-1$ s-keys). BM\&S works the same as M\&S, but with one difference in the recursive step where instead of merging all the s-nodes that are overfull, if any s-node is overfull, BM\&S merges exactly one s-node that has the largest size (i.e. $\arg\max_i |P_i|$, based on the notation in Section \ref{sec:merge:merge}), but BM\&S only merge down at most $s-f$ r-keys of $P_i$, if it has more. The recursive and split steps work as before, but this time there is at most one recursive call in each BM\&S operation.

BM\&S satisfies the new requirement on the maximum number of r-keys in non-leaf sibling s-nodes, because each level receives $s-f$ r-keys and flushes down $s-f$ r-keys if any of the sibling s-nodes has more than $s-f$ r-keys, and the requirement is already satisfied if none of the sibling r-keys has more than $s-f$ r-keys. Note that for leaf s-nodes we still perform splits if their size surpasses $s$ r-keys. Moreover, we can observe that the total size of siblings is at most $f\times s$.

\textit{Time Complexity.} Each BM\&S call performs at most $O(\log_{f}\frac{N}{s})$ number of Merge Down and Update and Split steps across all levels of the NB-tree. Each Merge Down as well as each Update and Split step take $O(\frac{fs}{B})$ page I/Os. As a result, the total time needed to perform one BM\&S function call, called on the root node is $O(\log_{f}\frac{N}{s}(\frac{fs}{B}\TSeqW + f\TSeek))$. We can perform $\frac{1}{s-f}$ of the $O(\log_{f}\frac{N}{s}(\frac{fs}{B}\TSeqW + f\TSeek))$ operations every time a new element is inserted into the root s-node. This results in BM\&S being finished by the time the root s-node is full again, and we can achieve the worst-case insertion time $O(\log_{f}\frac{N}{s}(\frac{fs}{B}\TSeqW + \frac{f}{s}\TSeek))$. The amortized insertion time in this case is the same as the worst-case insertion time. %Note that this is the same as the amortized insertion time for M\&S (but as shown above, the worst-case cost is improved from linear in $N$ to logarithmic in N).

\textit{BM\&S in the Background and Insertion Delay.} Note that when the root s-node becomes full, we can run BM\&S in the background, that empties the root s-node, and continue performing insertions in the emptied root s-node in the foreground. As long as the main memory s-node has space, the insertions will not make any disc accesses and therefore can be performed while the BM\&S operation is working in the background (performing queries  while BM\&S is running in the background is discussed in Section \ref{sec:concurrency}). This can reduce insertion delay significantly.

\if 0
Based on this, we can formulate what insertion rates the data structure can support. Recall that for a data structure to be able to support a certain insertion rate, $r$ ins./sec, it has to guarantee that delayed insertion time for all insertions into the data structure is zero. For this to be true in BM\&S, we need to show that when a BM\&S procedure is started after the in-memory s-node of an NB-tree becomes full, it will be over before the next time the in-memory s-node becomes full, so that new elements arriving can always be inserted in main memory without having to wait for the previous BM\&S call to be over. This is the subject of the theorem below. Note that here we are assuming in-memory insertion time is always less than $\frac{1}{r}$. 

\begin{theorem}\label{thm:rateGuarantee}
	An NB-tree can support insertions of rate $r$ if $r$ is $O(\big[\log_{f}\frac{N}{s}(\frac{f}{B}\TSeqW + \frac{1}{s}\TSeek)\big]^{-1})$. 
\end{theorem}
\fi

%Finally, note that the in-memory insertions need to be performed while BM\&S is emptying the memory. If the above inequality holds, elements leave the main memory faster than they arrive, and therefore the size of the data in main memory will not surpass $s$.

%On a technical detail, note that if the insertion rate $r$ satisfies the above inequality, when BM\&S is called on the root s-node, the rate at which BM\&S removes data from the main memory (to empty the root s-node) will be faster than $r$. Therefore, we can continue the insertions right after we call BM\&S without having to wait for the s-node to be entirely emptied, and still be sure that the size of the s-node will not surpass $s$ keys (typically, we can have a separate buffer s-node in memory to avoid the new in-coming r-keys getting mixed with the r-keys being moved down, but the total size will still be at most $s$ keys). 

\textit{Query Analysis.} Note that the maximum size of a node is $fs$ because that is the maximum total size of sibling s-nodes together. Thus, the query cost is now be at most $O(\log_B(fs)\times (\log_f(\frac{N}{s})))$ based on an analysis similar to Section \ref{sec:design:query}, but by changing the maximum size of a node. Note that $f$ is at most some fraction of $s$ and thus $\log_B(fs)$ is  $O(\log_B(s^2))$ which is $O(\log_B(s))$ and as a result we can write the query cost as $O(\log_B(s)\times (\log_f(\frac{N}{s})))$, which is asymptotically the same as before. 

\subsection{Concurrency of Queries and Merging}\label{sec:concurrency}
Recall that during the BM\&S operation, we never overwrite any parts of the data structure and we right the result of every step of the operation in a new location. Now consider merging the in-memory s-node, $T_0^0$, with its children $T_1^0$ to $T_1^k$. In the BM\&S operation, we first merge the r-keys in-memory with $T_1^0$ and move to the next child until $T_1^k$. Let ${T_1^i}'$ be the result of the merge of $T_0^0$ with $T_1^i$. Then, while writing ${T_1^i}'$, instead of waiting until the end of the procedure, we keep track of the root of ${T_1^i}'$  and write its location to $T_0^0$ while it is being updated (note that we can do this for ${T_1^i}'$ because its parent is the in-memory component and it incurs no extra page access, but we omit further implementation details here). This implies that while and after flushing down of $T_0^0$ is finished (before the recursive step of BM\&S), all the data in can be accessed from root and going through ${T_1^i}'$ for some $i$ (note that the pointers at the second level are not modified at all). Thus, performing queries during the recursive call step of the algorithm can be easily handled without any effect of the ongoing M\&S operation (as none of the data is overwritten). Finally, after the recursive calls, the ${T_1^i}'$ s-nodes will now need to be rewritten again (to update their pointers). This time, we will wait until the entire operation is finished and then update the pointers from $T_0^0$ to its children.







==> Old/Optimality.tex <==
\section{Performance Optimality}\label{sec:opt:opt}
As we have mentioned before, there is a trade-off between the query and insertion performance of different data structure. Thus, to compare two data structures, we need to consider the case when one of the two measures are the same and compare the other. The same applies when discussing the optimality of the performance of a data structure. Here, we will show that under certain conditions, and given a query cost requirement, no other data structure can provide an insertion time asymptotically lower than NB-trees in our comparison based external memory model. For this we first provide the following lemma.

\begin{Lemma}\label{lemma:optCost}
	Consider the case when the insertion cost for inserting $S$ elements to a comparison based external memory dictionary is $C_I$ and the data structure uses I/Os $C_Q$ to answer the queries in the worst-case, when $C_I$ is $\Omega(\frac{1}{B}\log^{1+\epsilon_1}S)$, for a constant $\epsilon_1>0$. Then, there exists a parameter setting for an NB-tree such that if an NB-tree uses $O(C_I)$ I/Os for the insertions, it will use $O(C_Q)$ I/Os to perform the query, if $B\geq \log^{3+\epsilon_2}N$ for a constant $\epsilon_2>0$.
\end{Lemma}
\textit{Proof.} Based on \cite{BF 03}, the statement of the lemma holds for $B^\epsilon$-trees. %TODO: double check
To show that it also hold for NB-trees, note that for any choice of $\alpha$ and by setting the branching factor of an NB-tree to that of $B^\epsilon$-tree, both its query and insertion cost becomes the asymptotically the same as a $B^\epsilon$-tree. Therefore, it means the statement is also true for NB-trees.

\hfill\ensuremath{\square}

Using the above lemma, we can provide the following theorem.

\begin{theorem}
	If an NB-tree performs queries using $O(C_Q)$ I/Os and takes time $O(T_I)$ seconds to perform $S$ insertions into the data structure, any other comparison based external memory dictionary that in the worst-case performs queries using $C_Q$ I/OS will take $\Omega(T_I)$ second to perform the insertions, for the case when the insertion cost is $\Omega(\frac{1}{B}\log^{1+\epsilon_1}S)$ and $B\geq \log^{3+\epsilon_2}N$ for constants $\epsilon_1, \epsilon_2>0$.
\end{theorem}
\textit{Proof.} Let $C_I$ be the cost of the insertions in an NB-tree that performs the queries in $O(C_Q)$. Based on Lemma \ref{lemma:optCost}, any other data structure must perform $\Omega(C_I)$ I/Os for the insertions as well. Note that the I/Os will at least take $\TSeqW$ time, thus the time will at least be $\Omega(C_I)\TSeqW$. Furthermore, at least, any data structure will perform $\Omega(\frac{S}{M})$ number of seeks ($M$ is the number of elements that can fit in memory), because any data structure has to write the $S$ elements to the disk at most $M$ elements at a time (and each write incurs at least 1 seek). Thus, any data structure will have to take time $\Omega(C_I\TSeqW + \frac{S}{M}\TSeek)$.

Based on the analysis in Section \ref{sec:opt:constSeek}, an NB-tree will perform $O(\frac{S}{S_n - f})$ seeks which is $O(\frac{S}{S_n})$ (assuming $f$ is at most a constant fraction of $S_n$). Setting $S_n = M$ will result in the minimum possible number of seeks and will only affect the query time by a constant factor. In this case, the insertion time, $T_I$, for an NB-tree will be $O(C_I\TSeqW + \frac{S}{M}\TSeek)$ which proves the theorem.

\hfill\ensuremath{\square}






==> Old/SSD.tex <==
\section{SSD}\label{sec:ssd}
Although our analysis mainly has focused on Hard disks, NB-trees can be utilized in SSDs as well, since reducing the number of seeks and performing sequential disk operation is also beneficial in SSDs. However, there are a number of other factors that can affect performance of a data structure in SSDs. Namely, as utilized in \cite{LHY+10} for their design, SSDs can perform multi-page I/Os, and moreover, random I/Os on SSDs within a small area (512KB-8MB) have a comparable performance to sequential ones.

These properties can be utilized in NB-trees to perform better in SSDs. For instance, setting the size of s-nodes to a value that can enjoy good locality, we can modify our merge policy to perform in-place B$^+$-tree insertions of the parent r-keys into the child's s-node, instead of reading the entire child's s-node and merging it with the parent. This would mean that each merge will take $O(s\log_B s)$ I/Os (because there will be at most $s$ B$^+$-tree insertions). This can be done in SSDs, despite the fact that they are random I/Os, because they are performed in a small area and thus they can take as low as sequential ones. It is not hard to see that (using proper buffering techniques) this method may perform less I/Os and still obtain a very low seek time. More importantly, the worst-case insertion cost will now be $O(\log_B s \log_f N)$, which now means than increasing $f$ can enhance both insertion and query cost (although it still need to be much smaller than $s$ to provide low number of seeks). 

%We do not go deeper in how to adopt NB-trees for SSDs, but various properties of SSDs can allow for better performance of NB-trees on SSDs compared with HDDs. 






==> Old/constantAmortizedSeek.tex <==
\section{Constant Amortized Number of Seeks}\label{sec:opt:constSeek}
Recall that based on our analysis in section \ref{sec:NB:I:T}, our data structure performs $O(\frac{1}{\alpha\epsilon B^{\alpha}}\log_BS)$ amortized number seeks. We can in fact reduce this to $O(1)$, by making some modifications to our merge procedure.

\subsection{Upgraded Merge and Split Procedure.} Based on the merge procedure discussed in Section \ref{sec:merge:merge}, we previously merged a node with its children right after the node becomes full. Here, instead, we will perform a merge when the total size of the nodes in a level goes above the sum of the maximum threshold for all the nodes in that level. That is, for the $i$-th level of the tree that includes $f^i$ nodes, we will perform the merge procedure if the total size of the nodes in that level goes above $f^i\times S_n$. When this happens, we read all the nodes in that level and merge them with the nodes in the level below it. However, instead of splitting the nodes as before, we will do upward propagation after the merge, as described below.

Furthermore, we change the requirement that every non-leaf outer node in an NB-tree has to have between $\frac{f-1}{2}$ to $f-1$ placed elements to the requirement that for every non-leaf level $i$, there has to be exactly $f^{i+1}-1$ placed elements. This might implies that some of the \BPTree nodes might not have any placed elements, which can be handled by minor modifications to how the pointers are set in each leaf node of the \BPTree, which we leave for the reader.

Assume that the $i$-the level of the tree is full (i.e. has at least $S_n\times f^i$ elements). To merge the $i$-th level with the $(i+1)$-th level (if the $i$-th level is the leaf level, we will perform the merge as explained before, but we assume that the $(i+1)$-th level is completely empty), we will read both of the levels sequentially from the disk, and write the merge output sequentially into a new location, but we will only merge $S_n\times f^i$ items of the $i$-th level and leave the rest of the items in that level untouched. We will read both levels page by page, find the smallest item between the two (they are both sorted so a procedure similar to the merge step of merge sort will be used) and insert the item into the newly created \BPTree that includes the merge output. We will treat all the elements of the $i$-th level as buffered elements in this procedure, but the placed elements of the $(i+1)$-th level will still remain as placed elements. Let the size of the $i$-th level before the merge be $s_i$, then when the size of the output \BPTree reaches $\frac{s_{i+1}+S_n\times f^i}{f^{i+1}}$, we will create a new \BPTree and continue with the merge. Note that this way, the updated $(i+1)$-th level will include exactly $f^{i+1}$ \BPTree nodes that are all (except the last one) of equal size. Furthermore, like before, we will keep the inner nodes of the \BPTree nodes full (i.e. of size $B$).

After the merge is completed, we will check whether the $(i+1)$-th component is full or not. If it is, we will merge it down with the next level using the same procedure. Otherwise, we perform the upward propagation on the $(i+1)$-th level as follows. We will read sequentially the $(i+1)$-th level, together with the $i$-th level (there will always be items left in the $i$-th level because it was overfull before the merge). For each \BPTree node in the $(i+1)$-th level (except the first node, i.e. the node that contains the smallest elements), we remove the smallest element of each \BPTree and merge the values with the $i$-th level, by writing it into a new location, where we now create new  \BPTree nodes of size $\frac{s_i - S_n\times f^i +f^{i+1}}{f^i}$ for the $i$-th level. All the elements that where already in the $i$-th level will be considered as buffered elements, while the elements that are moved up from the $(i+1)$-th level will be placed elements. When the upward propagation from the $(i+1)$-th level to the $i$-th level finishes, we move on to perform upward propagation from the $i$-th level to the $(i-1)$-th level. This continues until the level created from the upward propagation only contains one \BPTree node, which will be the root of the NB-tree and will be stored in the main memory. Note that as a result of the upward propagation from the $(i+1)$-th level to the $i$-th level, the $i$-th level will have exactly $f^{i+1}-1$ placed elements and exactly $f^{i}$ \BPTree nodes of equal size.

\subsection{Analysis}
First, we will discuss how the merge procedure will allow the queries to be performed as before. To see this, let the lowest level of the tree that the merge procedure merged down some data to it from the previous level be $l$. Note that the placed elements of the $l$-th level of the tree are not changed, so if the item to be queries is after the $l$-th level, we need to find the smallest placed element larger than the query value in the $l$-th level and follow its pointer. It is easy to verify that searching the data structure will reach the correct node of $l$, since a placed element for each node of the $l$-th level was inserted into the level above $l$. Note that, for the correctness of the query, it is essential that pointers in the leaf level of the nodes of an NB-tree are inserted correctly, using the procedure discussed in Section \ref{sec:NBTreeDesign}. 

Besides the correctness of the query, we need to show that the merge procedure will make sure no level of the tree is overfull. For this, we provide the following lemma.

\begin{Lemma}\label{lemma:Umerge:size}
	Assume that no level of an NB-tree is overfull before an insertion which results in the the root of the tree becoming overfull, and the tree's $i$-th level has at most $f^{i+1}$ placed elements for all $i$. After the merge procedure described above is finished, no node will be overfull. Furthermore, the $i$-th level will have at most $f^{i+1}$ placed elements for all $i$.
\end{Lemma}

\textit{Proof.} We will use an inductive argument to show that after the merge and upward propagation are over, the $i$-th level will have at most $S_n\times f^i$ elements. To see this, let the lowest level of the tree that the merge procedure merged down some data to it from the previous level be $l$. First note that the $l$-th level will have at most $S_n\times f^l$ elements, because the merge stopped there. Now assume that the induction hypothesis is true for $i+1$-th level. Then for the $i$-th level of the tree that moved some of its data down the tree (that is for $i<l$ and also $i\neq 0$), exactly $S_n(f^{i-1})$ elements where inserted into the level (from merging the $i-1$-th level with the $i$-th level) and at most $f^{i+1}$ elements where inserted into the level from the upward propagation of the $(i+1)$-th level (because of the induction hypothesis). This is while the level at most had $S_n(f^i)$ elements before the merge and exactly $S_n(f^i)$ where moved down from the level after the merge. Thus, the number of elements in the $i$-th level of the tree will at most be $S_n(f^{i-1})+S_n(f^i)-S_n(f^i)+f^{i+1}$. Assuming $f$ is at most $S_n-2$ and $S_n$ is at least equal to 4, the size will be at most $S_n(f^i)$ for $i>0$. For $i=0$, it's size will be at most $f+1$ because the merge starts when the size of the root is $S_n+1$. The merge moves $S_n$ elements down from the root, and move up to the root at most $f$ elements (because for any $i>0$ the $i$-th level won't be overfull).

Finally, note the number of placed elements in the $i$-th level is at most equal to the number of the nodes in the $(i+1)$-th level. The $(i+1)$-th level will have at most $f^{i+1}$ nodes by construction, which proves the lemma.

\hfill\ensuremath{\square}

Note that following the merge procedure, the query cost of the data structure will be the same, since the maximum size of each node has not changed. Next, we will discuss the amortized insertion time of the algorithm.

Observe that the merge procedure is called every time the root of the NB-tree becomes full, which is at most $\frac{S}{S_n-f}$ times. Also note that for every merge, for the $i$-th level of the tree, exactly $S_n\times f^i$ elements are moved down and at most $f^{i+1}$ elements are moved back up (because of upward propagation). Which means the net amount of data moved down is at last $S_n\times f^i - f^{i+1}$. Note that the data is moved down only during the merging process. Since by the end of the insertions, at most all the data has been move down from the $i$-th level, then the merge must have reached the $i$-th level at most $\frac{S}{S_n\times f^i - f^{i+1}}$ times. This also implies that at most $\frac{S}{S_n\times f^i - f^{i+1}}$ times the lowest level the merge processes reaches is the $i$-th. If the lowest level of the tree the merge processes reaches is the $i$-th level, the cost of merging will be equal to reading and writing all the levels of the tree up to the $i$-th level. Thus, the total cost of merging will be at most the sum, over all levels $i$, of the cost of the merge process when the lowest level reached is the $i$-th level. In other words

$$
O(\sum_{i=0}^{log_f S} \frac{S}{(S_n-f)\times f^{i}}\frac{S_n}{B}(f^{i+1} +f^i+...+1))
$$

Note that $f^{i+1} +f^i+...+1$ is $O(f^{i+1})$. Thus we can simplify the equation to

$$
O(\frac{S\times S_n}{(S_n-f)\times B}\sum_{i=0}^{log_f S} \frac{f^{i+1}}{f^i})
$$

Which can be written as 

$$
O(\frac{S\times S_n\times flog_f S}{(S_n-f)\times B})
$$

Thus, the amortized cost of insertion will be $O(\frac{S_n\times flog_f S}{(S_n-f)\times B})$. Same as before, assuming $f$ is at most a constant fraction of $S_n$, we can write the amortized cost as $O(\frac{f}{B}log_f S)$. Similar to the analysis in Section \ref{sec:NB:I:T}, letting $f=B^{\alpha\epsilon}$, the insertion cost will be $O(\frac{1}{\alpha\epsilon B^{1-\alpha\epsilon}}log_f S$, which is the same amortized cost as the previous merge procedure discussed. 

To find the amortized insertion time, note that if a merge procedure reaches at most the $i$-th level of the tree, it will perform $O(i)$ number seeks (each level is read twice and written once). This means that the total number of seeks performed in the merge operation will be 

$$
O(\frac{S}{(S_n-f)}\sum_{i=0}^{log_f S} \frac{i}{f^i})
$$

Note that $\sum_{i=0}^{\inf} \frac{i}{f^i}$ is $O(1)$ for any $f$ at least equal to 2. Thus, the total number of seeks will be $O(\frac{S}{S_n-f})$. Thus the amortized insertion time will be 

$$
O(\frac{flog_f S}{B})\TSeqW + O(\frac{1}{S_n-f})\TSeek
$$

Note that $O(\frac{1}{S_n-f})$ is $O(1)$, thus the algorithm performs constant amortized number of seeks.



==> Old/design.tex <==

%Finally, each s-node contains at most $f-1$ \textit{structural keys}, or in short, \textit{s-keys}. S-keys are special keys because each s-key is associated with a \textit{structural pointer}, or in short, \textit{s-pointer} that points to an s-node in the next level of the s-tree. An s-node that is pointed to by an s-pointer is the child of the s-node containing the s-pointer. The \textit{last child} of an s-node is the child of the s-node that contains the largest key. In Fig. \ref{fig:NBTreeExampleInsert} (g), the s-node $N_1$ contains 2 s-keys, i.e., the keys 15 and 49 shown in black. Both keys are associated with s-pointers, i.e., $L_1$ and $L_3$, where $L_1$ points to the s-node $N_2$ and $L_3$ points to the s-node $N_3$. Each s-node can also contain several other s-pointers (such as $L_2$, $L_4$ and $L_5$ in Fig. \ref{fig:NBTreeExampleInsert} (g)), whose purpose is discussed later. In Fig. \ref{fig:NBTreeExampleInsert} (g), $N_2$, $N_3$ and $N_4$ are children of $N_1$, and $N_4$ is the last child. 

%Now, consider an s-node. The s-node contains a B$^+$-tree with a few modifications only at the leaf level, referred to as a \textit{data tree} or in short, \textit{d-tree}, and we refer to the nodes in a d-tree as \textit{data nodes} or \textit{d-nodes}. In Fig. \ref{fig:NBTreeExampleInsert} (g), $M_{1, 1}$, $M_{1, 2}$,  $M_{1, 3}$ and $M_{1, 4}$ are d-node that together form a d-tree in the s-node $N_1$. 

%A d-tree maintains all the properties of a B$^+$-tree with fanout $B$, which we briefly mention here. The non-leaf d-nodes contain at most $B-1$ keys and $B$ pointers to their children and, except for the root, they contain at least $\lceil\frac{B}{2}\rceil$ keys and $\lceil\frac{B}{2}\rceil+1$ pointers. In Fig. \ref{fig:NBTreeExampleInsert}, $B$ is set to 5, and each d-node can have at most 5 children. In Fig. \ref{fig:NBTreeExampleInsert} (g), $R_1$, $R_2$ and $R_3$ show the pointers from a non-leaf d-node to its children. The leaf level d-nodes contain the keys in a sorted order, and each key is associated with a \textit{value} written next to it that contains the relevant data for each particular key. At the end of each leaf d-node there is a pointer, called \textit{sibling pointer}, to the next leaf d-node, following which the keys can be retrieved in the sorted order. $S_1$ and $S_2$ are such pointers in Fig. \ref{fig:NBTreeExampleInsert} (g). Moreover, for a non-leaf d-node with $q$ keys, say $K_1$, $K_2$, ..., $K_q$, the d-node pointed to by the $i$-th pointer $P_i$, $1< i\leq q$, contains keys $K$ such that $K_{i-1}\leq K < K_i$. For $i=1$, it only holds that $K< K_1$ and for $i = q+1$ it holds that $K\geq K_q$.

%However, for leaf d-nodes in non-leaf s-nodes, there are two additions to the traditional B$^+$-tree structure in a d-tree. First, as mentioned previously, each s-key contains an s-pointer written next to it (s-keys only exist at the leaf level of d-trees), we call this s-pointer an \textit{s-key s-pointer}. Secondly, each leaf d-node also contains an s-pointer written at the end of the d-node (next to the sibling pointer), which we refer to as \textit{d-node s-pointer}. A d-node s-pointer follows the property, referred to as the \textit{d-node s-pointer property}, that for a d-node, $M$, a d-node s-pointer points to the same s-node as the s-key s-pointer of the next s-key encountered when the keys are traversed in a sorted order starting from the d-node pointed to by the sibling pointer of $M$. If no such an s-key exists after the traversal, the d-node s-pointer will point to the last child of the s-node.  In Fig. \ref{fig:NBTreeExampleInsert} (g), $L_2$, $L_4$ and $L_5$ are d-node s-pointers, while $L_1$ and $L_3$ are s-key s-pointers. Observe that $L_2$ points to the same s-node as $L_3$, which is the first s-key encountered when traversing the d-nodes using $S_1$. However, no s-key is encountered when traversing the d-nodes from $S_2$, so $L_4$ points to the last child of $N_1$, which is $N_4$. Similarly, $L_5$ points to $N_4$, because there are no more d-nodes to traverse after the end of $M_{1, 4}$.

%Finally, we refer to the keys in a d-node that are not an s-key as \textit{regular keys} or \textit{r-keys}. For example, in d-node $M_{1, 3}$ in Fig. \ref{fig:NBTreeExampleInsert} (g), keys 26 and 47 are r-keys.

%As mentioned previously, there are two types of keys in an NB-tree, r-keys and s-keys. Any new key that is inserted into an NB-tree is an r-key, and some of the existing r-keys will be converted into s-keys during the \textit{oversized s-node handling operation} triggered by the insertion operation. 

%There are four operations that are the building blocks of NB-tree insertions, called \textit{s-node insertion}, \textit{r-key downward flushing}, \textit{s-node split} and \textit{oversized s-node handling}. We first discuss these operations separately and then move on to discuss the insertion operation itself.

%\textbf{S-Node Insertion.} Here, we discuss how a key-value pair $(K, V)$ is inserted into an s-node $N$. The insertion is similar to a B$^+$-tree insertion, but we need to preserve the cross-s-node linkage and the d-node s-pointer property. %(due to the existence of s-key s-pointers and d-node s-pointers). Consider Figure \ref{fig:NBTreeExampleInsert} (g). The d-tree in the s-node $N_1$ contains s-key s-pointers, namely $L_1$ and $L_3$, and d-node s-pointers, namely $L_2$, $L_4$ and $L_5$. 


%$SNodeInsert(N, K, V, P_{small}, P_{large})$ performs the insertion of an s-key or an r-key $K$ (with its value $V$) into an s-node $N$. If $P_{small}$ and $P_{large}$ are both $NULL$, then $K$ is an r-key. Otherwise, $K$ is an s-key and $P_{small}$ is the s-pointer associated with $K$, and $P_{large}$ is an s-pointer to the sibling of $N$ that contains the smallest key larger than keys in $N$. Since a d-tree is similar to a B$^+$-tree, the insertion is done in the same way as a B$^+$-tree insertions. 

%Next, we first describe the insertion operation of an r-key and then the insertion operation of an s-key. Consider performing an insertion of the r-key $K$ into the s-node $N$, $SNodeInsert(N, K, V)$. Note that $N$ contains a d-tree. First, we find the leaf d-node $M$ of the d-tree in which $K$ is to be inserted by a B$^+$-tree search and insert $K$ into $M$. If $M$ does not need to split, the insertion is finished. Otherwise, we split it in the same way as a B$^+$-tree split, into two d-nodes $M_{small}$ and $M_{large}$, where $M_{small}$ contains the smaller half of the keys and $M_{large}$ the rest, and $M_{small}$ and $M_{large}$ each has a d-node s-pointer and may contain s-keys. Next, we do some operations to maintain the d-node s-pointer property. We set the d-node s-pointer of $M_{large}$ to that of $M$. If $M_{large}$ does not contain any s-key, then the d-node s-pointer of $M_{small}$ will be set to the that of $M_{large}$. Otherwise, we set the d-node s-pointer of $M_{small}$ to the s-key s-pointer of the smallest s-key in $M_{large}$. 

%Now, consider performing the insertion of the s-key $K$ into an s-node $N$. The insertion of an s-key into $N$ only happens when a child, $C$, of $N$ has been split (we will describe the operation \textit{split} later) into two children $C_{small}$ and $C_{large}$. Consider two s-pointers $P_{small}$ and $P_{large}$ pointing to the two children respectively, which are obtained from the $split$ operation. We refer to this operation as $SNodeInsert(N, K, V, P_{small}, P_{large})$. First, we follow the same procedure as inserting an r-key into the s-node described above. After the insertion is finished, consider the leaf d-node, $M$ that contains $K$. Let $M_{small}$ be the leaf d-node containing the largest s-key in $N$ smaller than $K$, or the first leaf d-node of $N$ if there is none. Besides, let  $M_{large}$ be the leaf d-node containing the smallest s-key in $N$ larger than $K$, or the last leaf d-node of $N$ if there is none. Next, we do some operations to maintain the d-node s-pointer property. For all the leaf d-nodes along the (leaf-level) traversal starting from $M_{small}$ until, and not including, $M$, the d-node s-pointer of each of these leaf d-nodes will be set to $P_{small}$. Moreover, for all the leaf d-nodes along the (leaf-level) traversal starting from $M$ until, and only including $M_{large}$ if $M_{large}$ is the last leaf d-node of $N$, the d-node s-pointer for each of these leaf d-nodes will be set to $P_{large}$. If an s-key larger than $K$ exists in $N$, for the smallest s-key larger than $K$, we set its s-key s-pointer to $P_{large}$.

%For example, consider the root s-node, $N_1$, in Fig. \ref{fig:NBTreeExampleInsert} (f), which contains one d-node, $M_{1, 1}$. Consider inserting seven keys in $N_1$, namely 11, 24, 25, 26, 47, 55 and 61. The insertion is done in a B$^+$-tree manner, as shown in Fig. \ref{fig:NBTreeExampleInsert} (g), but it causes $M_{1, 1}$ to split (several times). When $M_{1, 1}$ splits and new d-nodes are created, their d-node s-pointer need to be set. In Fig. \ref{fig:NBTreeExampleInsert} (g), the d-node s-pointers $L_2$, $L_4$ and $L_5$ are set according to the d-node s-pointer property after the new keys are inserted in the d-tree of $N_1$. 

%For instance, based on the d-node s-pointer property, $L_2$ points to the same s-node (i.e., $N_3$) as the next s-key encountered when traversing the leaf d-nodes using the sibling pointer of $M_{1, 2}$, that is the s-key 49. Thus, $L_2$ points to the s-node that $L_3$ points to, i.e., to $N_3$. For both $L_4$ and $L_5$, since no s-key is encountered when traversing the leaf d-nodes, they point to the last child of $N_1$, which is $N_4$. Note that since the keys that are inserted into $N_1$ are r-keys, the s-key s-pointers in $N_1$ (i.e., $L_1$ and $L_3$) do not change. 

%The insertion of an s-key into an s-node is always triggered after r-key insertions. For instance, consider the case when the r-key 66 is inserted into the root s-node in Fig. \ref{fig:NBTreeExampleInsert} (e). This first results in $HandleFullSNode$ operation (to be described later) which consequently trigger the insertion of the s-key 49 into the s-node $N_1$, as shown in Fig. \ref{fig:NBTreeExampleInsert} (f). The insertion of the s-key into $N_1$ sets the s-key s-pointer of the s-key 49, as well as the d-node s-pointer of $M_{1, 1}$. Note that, in Fig. \ref{fig:NBTreeExampleInsert} (e),  the key 49 is an r-key that exists at the leaf level of the s-tree. However, after it is inserted into $N_1$ in Fig \ref{fig:NBTreeExampleInsert} (f), it is converted into an s-key (see \textit{Oversized S-Node Handling Operation} below for more details).

%\textbf{R-Key Downward Flushing.} For a non-leaf s-node $N$ that violates the size requirement, $flush(N)$ ensures that after it is called, $N$ does not violate the size requirement. The operation moves the r-keys in $N$ to its children. 

%Consider the list of s-keys in the s-node, $N$, that contains $q$ s-keys in a sorted order and assume that $K_i$ is the $i$-th s-key in that order, $1\leq i\leq q$, and that $P_i$ is the s-key s-pointer of $K_i$. Now, consider an r-key $K$ in the s-node. For each r-key $K$, where $K_{i-1}\leq K < K_i$, the $flush$ operation removes $K$ from the s-node, $N$, and inserts it in the s-node pointed to by $P_i$. If $K < K_1$, then it is inserted into the s-node pointed to by $P_1$ and if $K\geq K_q$, it is inserted into the last child of the s-node $N$. The insertion of each r-key into a child s-node is done using the $SNodeInsert$ operation. Note that after the $flush$ operation, the d-node s-pointers in $N$ need to be re-adjusted similar to how its done in $SNodeInsert$ to satisfy the d-node s-pointer property. Finally, we can only flush down a specified number of r-keys from $N$, and leave any more existing r-keys in $N$ without moving them to its children. The specified number will be described later.

%For instance, in Fig. \ref{fig:NBTreeExampleInsert} (g), if a $flush$ operation is called on $N_1$, it will move 11 to $N_2$, 24, 25, 26 and 47 to $N_3$ and 55 and 61 to $N_4$ and removes all the r-keys from $N_1$. After a $flush$ operation, $N_1$ will only contain s-keys 15 and 49.

==> Old/designBack.tex <==
\section{Design of Nested B-tree}\label{sec:NBTreeDesign}
%In this section, we provide a data structure that achieves an asymptotically optimal read performance while supporting fast insertions on large volumes of data. We propose Nested B-trees or NB-trees for short. Intuitively, an NB-tree is a B-tree whose nodes are B$^+$-trees, and the newly inserted data is buffered in the B$^+$-tree of each of the nodes and moves down the tree when the B$^+$-tree in a node is full.

\subsection{Definition and Properties}
In the following, we propose a novel indexing structure called the \emph{nested B-tree} (or in short, \emph{NB-tree}), that achieves an asymptotically optimal read performance while supporting fast insertions on large volumes of data. An NB-tree involves two types of trees. The first type is called an \emph{structural tree} (or \emph{s-tree}) and the second is called a \emph{data tree} (or \emph{d-tree}).

\subsubsection{Definitions.} In the entire NB-tree, there is exactly one instance of the structural tree and multiple instances of the data tree. The \emph{structural tree} (or s-tree) contains a set of nodes called the \emph{structural nodes} (or in short, \emph{s-nodes}). Each s-node in the s-tree is a \emph{data tree} (to be described in detail later). Like a normal tree data structure, the s-tree, has one \emph{root s-node} and other \emph{non-root s-nodes} and an s-node in the lowest level of the s-tree, is called a \emph{leaf s-node}. Each non-leaf s-node has at most $f$ child s-nodes where $f$, a positive integer,  is called the \emph{fanout} of the s-tree. We number the levels in an s-tree, starting from the root s-node, which is at \emph{Level 0}. All children of the root s-node are at \emph{Level 1} and the remaining levels are numbered similarly, with $l_{max}$ being the greatest level number. Let $T_i$ be the set of s-nodes in the s-tree at level $i$, $i \in [0, l_{max}]$. $T_i$ contains $|T_i|$ s-nodes, namely $T_i^1, T_i^2, ..., T_i^{|T_i|}$, where $T_i^j$ is the $j$-th node at Level $i$ of the s-tree.

\begin{example}
Consider an example of an NB-tree as shown in Figure~\insFigNo(g).
In this figure, the structural tree contains 4 s-nodes, namely $N_{1}, N_{2}, N_{3}$ and $N_{4}$, and $N_{1}$ is at Level 0 and other s-nodes
are at Level 1 of the structural tree.
$N_{1}$ is a root s-node and $N_{2}, N_{3}$ and $N_{4}$ are leaf s-nodes.
%
Each s-node corresponds to a data tree (illustrated in detail later).
\end{example}

A \emph{data tree} is a tree containing a set of nodes called the \emph{data nodes} (or in short, \emph{d-nodes}). Each d-node in a data tree stores a combination of \emph{pointers}
and \emph{key}-\emph{value} pairs.
Here, in a key-value pair, the \emph{value} in this pair corresponds to the whole data to be stored (or its disk pointer pointing to this whole data on a disk in case of an indexing data structure)
and the \emph{key} in this pair corresponds to the attribute to be indexed.
%Key-value pairs have different meanings in different contexts.
%In the context of indexing the records in a database on an attribute $A$,
%the disk pointer, pointing to a record on a disk, corresponds to a value; and
%the value of attribute $A$ of this record corresponds to a key.
%
%In the context of a typical key-value data store storing a list of key-value pairs,
%the key-value pairs in the list are exactly the key-value pairs in our context.
%For clarity, we focus on the first case.
%
%In case of a typical key-value data store storing a list of key-value pairs,
%the key-value pairs in the list are exactly the key-value pairs in our context. That is,
%each key-value pair in our context has a key component and a value component
%such that the value component corresponds to the data that is associated with that key.
%In case of an indexing data structure, each key-value pair has a key component and each value contains a pointer to the disk location where the actual data is written. In this paper, we focus on the second case for clarity.
%The theoretical
%analysis to be studied in this paper
%applies to both contexts,
%but with the difference that the size of the value entries/components in a key-value data store can be different for different pairs and can be very large, which complicates the theoretical complexity analysis.
%
In what follows, for clarity, we assume that NB-trees are used as an indexing data structure and that all key-value pairs are of a fixed size, and are small enough to allow multiple pairs to be stored on a disk page.

In Figure~\insFigNo(g), the tree within the entire $N_1$,
is the data tree. In this data tree,
there are four d-nodes, namely $M_{1, 1}, M_{1, 2}, M_{1, 3}$
and $M_{1, 4}$. $M_{1, 1}$ are at Level 0
and the other d-nodes are at Level 1 of this data tree. $M_{1, 1}$ is a root d-node and $M_{1, 2}, M_{1, 3}$ and $M_{1, 4}$ are leaf d-nodes.




\subsubsection{d-node Format.}\label{sec:design:format} S-tree and s-nodes are abstract notions, conceptually representing how different d-nodes are related, but only d-nodes are physically written on the hard disk. Next, we discuss what is stored at each d-node depending on its level in the s-tree and its corresponding d-tree.

\textit{Non-leaf d-nodes (in Either a Leaf s-node or a Non-Leaf s-node).} In this case, the d-node is in the form of $(P_1, K_1, P_2, K_2, P_3, K_3, P_4, ..., K_{n}, P_{n+1} )$ where $P_i$ a single pointer for $i \in [1, n+1]$ and $K_i$ is a single key for $i \in [1, n]$.
%$n$ has to satisfy the size requirements to be discussed in Section \ref{sec:design:size} that determines how many children the d-node has.
In Figure~\insFigNo(g),
since $N_1$ is a non-leaf s-node of the s-tree,
$M_{1, 1}$ is a non-leaf d-node in a non-leaf s-node.
Since $N_2$ is a leaf s-node of the s-tree,
$M_{2, 1}$ is a non-leaf d-node in a leaf s-node.

\textit{Leaf d-nodes in a leaf s-node.} In this case, the d-node is of the form $(K_1, V_1, K_2, V_2, K_3, V_3, K_4, ..., K_{n}, V_n, P_{sibling})$. Similar to any B$^+$-tree structure, each d-node has an additional pointer space slot, $P_{sibling}$, called the \emph{sibling pointer space slot}, that contains a pointer to the sibling d-node of the d-node. Moreover, each key, $K_i$, will have a value, $V_i$, written next to it, instead of a pointer. %Same as before, $n$ has to satisfy the size requirements to be discussed in Section \ref{sec:design:size}.
In Figure~\insFigNo(g),
since $N_2$ is a leaf s-node of the structural tree,
$M_{2, 2}$ is a leaf d-node in a leaf s-node.

\textit{Leaf d-nodes in a Non-leaf s-node.} The d-node is of the form $(K_1, V_1, [P_1,] K_2, V_2, [P_2,] ..., K_{i},  V_{i},  [P_i,]... K_{n}, V_n, [P_n,] P_{sibling}, P_{s-node})$. In the above form,  $P_i$ 
is called the \emph{s-key pointer space slot} for each $i \in [1, n]$.
Each square bracket enclosing $P_i$ means that $P_i$ is optional depending on whether $K_i$ is an \emph{s-key}
(which will be described in detail later). If $K_i$ is an s-key, then $P_i$ will exist in the above form and we say that $K_i$ is associated with $P_i$. % the pointer associated with $K_i$.
Otherwise, $P_i$ will not exist in the above form. 
%Besides,
%zero or more keys in this leaf d-node (e.g., $K_i$ in the above form) is \emph{associated}
%with a pointer space slot $P_i$ called
For example, if $K_1$ is an s-key but both $K_2$ and $K_3$ are not,
then the form of this d-node is $(K_1, V_1, P_1, K_2, V_2, K_3, V_3, ..)$.
%
%This pointer space slot contains a pointer to
%the root d-node of a data tree corresponding to the s-node of the structural tree which is at one level larger than the current level of the s-node containing this d-node.
%an s-node in the next level of the structural tree.
Moreover, each leaf d-node always has an additional pointer space slot, $P_{s-node}$, called the \emph{s-node space slot}. We will discuss the significance of these pointers later. %an s-node in the next level of the structural tree. %$n$ has to satisfy the size requirements discussed in Section \ref{sec:design:size}.
In Figure~\insFigNo(g),
since $N_1$ is a non-leaf s-node of the structural tree at Level 0,
$M_{1, 2}$ is a leaf d-node in a non-leaf s-node.
Note that $M_{1, 2}$ has two pointers.% each pointing to the root d-node of a data tree
%corresponding to the s-node of the structural tree at Level 1 of the structural tree
%(i.e., one level larger than the current level of the s-node containing $M_{1, 2}$).

%We call $P_i$ the pointer associated with $K_i$.

%That is, a leaf d-node in a leaf s-node, is of the form  $(K_1, V_1, K_2, V_2, K_3, V_3, K_4, ..., K_{n}, V_n, P_{sibling})$ where $P_{sibling}$ is a space slot storing a single pointer to a d-node (which is a sibling node of this d-node), and $n$ is the number of of each key-value pair that can fit on a disk page. A leaf d-node in a non-leaf s-node is of the form $(K_1, V_1, K_2, V_2, K_3, V_3, ..., K_{s}, V_{s}, P_{s}, ... K_{n}, V_n, P_{sibling}, P_{s-node})$, where in this case, $K_s$ is a key that has an additional pointer $P_s$ to an s-node in the next level of the s-tree and $P_{s-node}$ is the space slot for another pointer to an s-node in the next level of the s-tree. Note that, for leaf d-nodes in non-leaf s-nodes, $n$ also depends on the number of extra pointers stored in the d-node and can vary from d-node to d-node (although there is a limit on the number of such pointers as discussed later).

%Similar to other indexing structures, in order to utilize each d-node as much as possible, we would like to fill up the d-nodes as much as possible. For this, we introduce the \emph{d-node size requirements} as follows. For the non-root s-nodes, all the d-nodes except the last d-node on each level of a d-tree, we ensure that all the space slots are full and that there is no space available to insert a new key in any of such d-nodes. There is no requirement on the last d-node of each level in this case. For the root s-nodes, we ensure that at least half of each d-node is full.

%In other words, each d-node has $f$ space slots for storing $f$ different pointers and $f-1$ space slots for storing $f-1$ different keys.
%
%Note that some space slots could be filled with pointers/keys and some may not. Besides, the first pointer space slot $P_1$ and the first key space slot $K_1$ must be filled.
%

%Finally, each d-node is of size at most $\mathcal{B}$ bytes and

 %We make sure that the data is written into a d-node from the left hand side such that when we traverse the d-node from the left hand side to the right hand side in a d-node, all keys, values and pointers are read before any empty space is reached.

%Based on the form of each d-node, we know that each d-node contains at most $B$ keys (which fill up space slots for keys). Similar to other indexing structures, in order to utilize each d-node as much as possible, we would like to fill up at least half keys of each non-root d-node. Thus, we introduce this \emph{size requirement} as follows. Each non-root d-node contains at least $\lceil \frac{f-1}{2} \rceil$ keys (which fill up space slots for keys).

\subsubsection{Size Requirements.}\label{sec:design:size}


In the NB-tree, it is required that each d-tree contains at most $s$ keys in the leaf level
where $s$ is a positive integer and
%A data tree contains at most $s$ keys where $s$ is a positive integer and
is called \emph{size of a data tree} or equivalently \emph{size of an s-node}. In a d-tree \emph{root d-nodes}, \emph{non-root d-nodes} and \emph{leaf d-node} are defined similar to a normal tree data structure. To optimize for disk accesses, a d-node is at most of size $\mathcal{B}$ bytes, where $\mathcal{B}$ is the disk page size. Similarly, each data tree has a number of levels, starting from Level 0.

Note that the size of an s-node can also be equivalently defined by the number of disk pages occupied by the s-node on a hard disk, but we use the above definition it allows for a simpler notation in the analysis, and that the maximum number of pages an s-node with $s$ keys occupies can be easily calculated based on the size requirements to be discussed below in this section. However, in practice, we can set the size of an s-node based on the maximum number of pages we want to allow an s-node to occupy. For instance, in our example in Fig. 2, we have set $s$ to be equal to 4 pages.


Similar to other indexing structures, in order to utilize each node as much as possible, we would like to fill up the nodes as much as possible. For this, we introduce the \emph{size requirements}. %Let the size of a disk pointer, key and value be $b_p$, $b_k$ and $b_v$ bytes, respectively. 
Let $B$ be the maximum number of keys stored in a leaf d-node and let $B'$ be the maximum number of keys stored in a non-leaf d-node (based on the discussion in Section \ref{sec:design:format}, values of $B$ and $B'$ can easily be calculated given the size of disk pointers, keys and values and the fact that each d-node is of size $\mathcal{B}$ bytes). Then, we impose the following size requirements on s-nodes and d-nodes in an NB-tree.

%We could obtain $B = \lfloor\frac{\mathcal{B}-2b_p}{b_k+b_v+b_p}\rfloor$ and $B'=\lfloor\frac{\mathcal{B}-b_p}{b_k+b_p}\rfloor$.
%Then, based on the discussion in Section \ref{sec:design:format}, and for a non-leaf d-node to be of size $\mathcal{B}$,
%we compute $B'=\lfloor\frac{\mathcal{B}-b_p}{b_k+b_p}\rfloor$, which means that
%a non-leaf d-node can have at most $B'$ keys and $B'+1$ child d-nodes.
%
%Similarly, we compute $B = \lfloor\frac{\mathcal{B}-2b_p}{b_k+b_v+b_p}\rfloor$
%since in the worst case, a leaf d-node can have at most $B$ keys to be at most of size $\mathcal{B}$ (note that depending on the number of pointers in a leaf d-node, it might be able to contain more than $B$ keys and still be of size at most $\mathcal{B}$, but for simplicity, we assume that it can have at most $B$ keys). Furthermore, since we are focusing on the context of indexing records, $b_v$ and $b_p$ are of the same size and therefore, $B'$ will be larger than $B$ within a constant factor. Then, we impose the following size requirements on s-nodes and d-nodes in an NB-tree.

\begin{itemize}
    \item \textit{d-node size requirements.}
    \begin{itemize}
       \item \textit{Root d-nodes.} Each root d-node has at most $B-1$ keys.
        \item \textit{Leaf d-nodes (which is not a root d-node).} Each leaf d-node has between $\lfloor\frac{B-1}{2}\rfloor$ and $B-1$ keys.
        \item \textit{Non-leaf d-nodes (which is not a root d-node).} Each non-leaf d-node has between $\lfloor\frac{B'-1}{2}\rfloor$ and $B'-1$ keys.
    \end{itemize}
    \item \textit{s-node size requirements.}
    \begin{itemize}
        \item \textit{Non-leaf or root s-nodes.} Each non-leaf s-node has between $1$ and $s$ number of keys.
        \item \textit{Leaf s-nodes (which is not a root s-node).} Each leaf s-node has between $\lfloor\frac{s}{2}\rfloor$ and $s$ number of keys, unless it is also a root.
    \end{itemize}

\end{itemize}

\subsubsection{The Tree Structure.} In a d-tree, each d-node stores keys. We classify the keys into two types, namely \emph{regular keys} (or \emph{r-keys}) and \emph{structural keys} (or \emph{s-keys}). In Figure~\insFigNo(g), all keys in the ``white'' color background (e.g., 1, 11 and 51) are r-keys and all keys in the ``black'' color background (e.g., 15 and 49) are s-keys. When s-key is stored in the key space slot $K_i$ of a leaf d-node,
it is associated with the s-key pointer space slot.
When r-key is stored, it is not associated with the s-key pointer space slot. Note that, the tree structure of an s-tree and d-trees is imposed by the pointers we have mentioned so far. Next, we discuss how each of the pointers are set. For this, Consider d-node in a data tree, $T_d$, corresponding to an s-node at Level $i$ of the s-tree.

%Each entire data tree contains at most $f-1$ s-keys. All remaining keys in the entire data tree are r-keys. s-keys only exist in the leaf d-nodes of a non-leaf s-node. %, and are defined as the keys in a leaf d-node that contain a pointer.

%$K_1$ is associated with a pointer space slot $P_1$
%
%That is, each s-key is associated with a pointer (the pointer is written next to the s-key in a leaf d-node, as describe in Section \ref{sec:design:format}) that points to an s-node in the next level of the s-tree.

%In the data tree, consider a leaf d-node in a non-leaf s-node. % stores a pointer in the pointer slot $P_{s-node}$.
%There are in total four types of pointers: (1) pointers associated with r-keys,
% (2) pointers in $P_{sibling}$ point from a d-node to another d-node in the same s-node,
% (3) pointers associated with s-keys,
% and (4) pointers in $P_{s-node}$ point from a d-node in an s-node to a d-node in another s-node. %That is, for a d-node in $T_d$,

\begin{itemize}
  \item If this d-node is a non-leaf d-node at Level $j$ where $j$ is  a non-negative integer, each of the pointers stored in this d-node is a pointer to one of the d-nodes at Level $j+1$ in the same data tree $T_d$. In Figure~\insFigNo(g), $M_{1, 1}$ at Level 0 has three pointers, namely $R_1, R_2$ and $R_3$ pointing to d-nodes at Level 1.
  \item If this d-node is a leaf d-node, $P_{sibling}$ stores the pointer to a d-node which is the next sibling d-node in $T_d$ (where the next sibling d-node has the same meaning as a B$^+$-tree). Figure~\insFigNo(g) shows that $M_{1, 2}$, a leaf d-node, has a space slot $P_{sibling}$ storing pointer $S_1$ pointing to its next sibling d-node $M_{1, 3}$.
      The other pointers stored in the d-node can be assigned under the following two sub-cases.
     \begin{itemize}
       \item If $i = l_{max}$ ($T_d$ is in a leaf s-node of the s-tree), the d-node does not store any pointers (other than $P_{sibling}$). As an example, see $M_{2, 2}$ in Figure~\insFigNo(g).
       \item If $i < l_{max}$ ($T_d$ is in a non-leaf s-node of the s-tree), in this d-node, each of the pointers (except $P_{sibling}$) is a pointer to the root d-node of the d-tree of an s-node of the s-tree at Level $i+1$. In this case, the pointer space slot $P_{s-node}$ stores a pointer as described above. Besides, if a key space slot $K_i$ is associated with the s-key space pointer slot, then the pointer space slot $P_i$ stores a pointer as described above.
           In Figure~\insFigNo(g), since $M_{1, 2}$ is a leaf d-node in the s-node at the non-leaf level of the structural tree, 
           the s-key space pointer slot in this d-node which corresponds to the s-node $N_1$ at Level 0 stores the pointer $L1$ pointing to the root d-node of the data tree which corresponds to the s-node $N_2$ at Level 1 of the structural tree.
           The d-node $M_{1, 2}$ has the space slot $P_{s-node}$ shown at the end of this node storing the pointer $L_2$ pointing to the root d-node of
           the data tree which corresponds to the s-node $N_3$ at Level 1 of the structural tree. 
     \end{itemize}
\end{itemize}

Moreover, we have the following requirement on the number of children of an s-node.

\begin{itemize}
    \item \textit{Structural Requirement.}
    \begin{itemize}
        \item Each non-leaf s-node has between $\lfloor\frac{f}{2}\rfloor$ and $f$ children and between $\lfloor\frac{f-1}{2}\rfloor$ and $f-1$ s-keys.
        If a non-leaf s-node is also a root s-node, then the lower limits are 2 and 1, respectively.
        \item The parameter $f$ is at most $\frac{s}{2}$.
    \end{itemize}
\end{itemize}

We impose the restriction on the maximum value of $f$ to provide a better insertion performance, as will be discussed in Section \ref{sec:design:insertion}.
However, the factor two in the upper bound mentioned above (i.e., $\frac{s}{2}$)
is arbitrarily chosen for concreteness. In fact,
the upper bound of $f$ can be set to any constant fraction of $s$.


\subsubsection{Properties.} A data tree has all the properties of a typical B$^+$-tree. For instance, all the data is stored in the leaf d-nodes and that traversing the leaf d-nodes from the left hand side to the right hand side retrieves all the data stored in the data tree in an ascending order. 

\if 0
\begin{itemize}
   \item \emph{Leaf-Level Ascending Property:}
        If we traverse all leaf d-nodes in $T_d$ from the left hand side to the right hand side, and iteratively traverse the next leaf d-node from the current d-node by following the sibling pointer of the current d-node, then all keys traversed are in ascending order.
        In Figure~\insFigNo(g), we could see that in the data tree in $N_1$, when we traverse from the left hand side to the right hand side in
        the leaf level, we have 11, 15, 24, 25, 26, 47, 49, 55 and 61 which is in ascending order.
   \item \emph{Leaf-Level Key Property:}
        All keys stored in all leaf d-nodes in $T_d$ contributes to all keys stored for $T_d$ (which corresponds to an s-node of the structural tree).
        Let $D(T_d)$ be the set of all these keys for $T_d$.
        In Figure~\insFigNo(g), if $T_d$ is the data tree in $N_1$, $D(T_d) = \{11, 15, 24, 25, 26, 47, 49, 55, 61\}$.
   \item \emph{Non-Leaf d-Node Property:}
      Note that the non-leaf d-node is in the form of $(P_1, K_1, P_2, K_2, P_3, K_3, P_4, ..., K_{n}, P_{n+1})$.
      \begin{itemize}
        \item Each key in $D(T_d)$ at most $K_1$ could be found in one of the leaf d-nodes of the sub-tree rooted at the d-node pointed by pointer $P_1$.
        In Figure~\insFigNo(g), consider d-node $M_{1, 1}$ in the data tree $T_d$.
        Consider key 15 in this d-node.
        We could see all keys in $D(T_d)$ at most 15 could be found in the leaf d-node $M_{1, 2}$ of the sub-tree rooted at the d-node pointed by pointer $R_1$
        \item For each pair $(K_i, K_{i+1})$ where $i \in [1, n-1]$, each key in $D(T_d)$ greater than $K_i$ and at most $K_{i+1}$ could be found in one of the leaf d-nodes of the sub-tree rooted at the d-node pointed to by pointer $P_{i+1}$.
        In Figure~\insFigNo(g), consider d-node $M_{1, 1}$ in the data tree $T_d$.
        Consider key 15 and key 49 in this d-node.
        We could see all keys in $D(T_d)$ greater than 15 and at most 49 could be found in the leaf d-node $M_{1, 3}$ of the sub-tree rooted at the d-node pointed by pointer $R_2$.
        \item Let $i'$ be the greatest index in $[1, n]$ such that $K_{i'}$ is non-empty.
        Each key in $D(T_d)$ grater than $K_{i'}$ could be found in one of the leaf d-nodes of the sub-tree rooted at the d-node pointed by pointer $P_{i'+1}$.
      \end{itemize}
\end{itemize}
\fi

Next we discuss the properties different from a typical B$^+$-tree. Note that each non-leaf s-node (or its corresponding data tree), $T_d$, has at least one s-key,
and satisfies the structural requirement. Each s-key is associated with the s-key pointer space slot storing a pointer to an s-node in the next level of the s-tree.
Let $K_{1}, K_{2}, K_{3}, ..., K_{n}$ be the list of all s-keys in the data tree where $K_1 < K_2 < ... < K_n$.
%It is easy to know that when we traverse all leaf d-nodes from the left hand side
%to the right hand side, if we just extract all s-keys, we will obtain this list of all s-keys.
%
In Figure~\insFigNo(g), in $N_1$, there are two s-keys, 15 and 49.
Then, in this example, $K_1 = 15$ and $K_2 = 49$.
%
For the ease of discussion, assume $T_d$ contains two fictitious s-keys, $K_0 = -\infty$ and $K_{n+1} = +\infty$ and a fictitious d-node containing $K_{n+1}$ (in the first position of the d-node) as an s-key,
where $P_{sibling}$ of the last (or rightmost) sibling d-node in the leaf level of $T_d$ to the pointer to this fictitious d-node. %Note that
%these two fictitious keys were not in our implementation. They are just for the illustration purpose.
%

%For simplicity, assume that $-\infty$ and $+\infty$ are stored as s-keys in all the s-nodes, where $+\infty$ has the same pointer as $P_{s-node}$ of the last d-node in the s-node (the pointer of $-\infty$ can by NULL). Consider, in $T_d$, the sorted list of s-keys $K_{1}, K_{2}, K_{3}, ..., K_{n}$ for an integer $n$ that satisfies the structural requirements ($K_{0}$ is $-\infty$ and $K_{n}$ is $+\infty$). Note that the s-keys may be stored in different d-nodes within the same s-node. Then, we have the following properties.

\begin{itemize}
   \item \emph{Cross-s-Node Linkage Property.}
   \begin{itemize}
       \item For two consecutive s-keys $K_{i-1}$ and $K_{i}$ where $i$ is an integer in $[1, n+1]$,
            each key in $D(T_d')$ is greater than $K_{i-1}$ and is at most $K_i$
            where $T_d'$ is the data tree with its root d-node pointed by $P_i$.
%
d-node $M_{1, 2}$ in Figure~\insFigNo(g) has an s-key, 15. The s-key space pointer associated with 15
is $L_1$ that points to the d-tree in $N_2$. All keys in $N_2$ (i.e., 1, 2, 3, 4, 5, 6, 7, 8, 9, 10 and 14)
are smaller than 15 and greater than $K_0 = -\infty$.            
       \item Consider a leaf d-node $N_d$.
            Consider traversing to the next sibling d-node $N_d'$ starting from $N_d$ (by following $P_{sibling}$)
            iteratively until we find $N_d'$ containing an s-key, $K_i$.
            Each key in $D(T_d')$ is greater than $K_{i-1}$ and is at most $K_i$
            where $T_d'$ is the data tree with its root d-node pointed by the pointer in the space slot $P_{s-node}$, which is the same as $P_i$.
%
Consider the leaf d-node $M_{1, 2}$ in Figure~\insFigNo(g).
The space slot $P_{s-node}$ of this leaf d-node which is shown at the end of this d-node stores pointer $L_2$ pointing to the data tree $T_d'$ in $N_3$.
Note that we could traverse from this d-node to the next sibling d-node $M_{1, 3}$ containing an s-key (i.e., key 49).
Here, $K_i = 49$. We also deduce that $K_{i-1} = 15$.
All keys in this data tree $T_d'$ (i.e., 16, 18, 20, 21, 29, 32, 33)
are greater than 15 and are at most 49, and that $L_2$ points to the same s-node as $L_3$.       
%
%       For a d-node $N_d$, let $K_{i}$ be the first s-key encountered when following $P_{sibling}$ and traversing the leaf d-nodes of the d-tree in ascending order from there (not including the $N_d$). Note that for $i$, it will true that $1\leq i\leq n$. Then, let the s-node pointed by $K_{i}$ be $T_d'$. Then, for all keys $K_j$ where $K_j\in D(T_d')$, we have that $K_{i-1}< K_j \leq K_{i}$.
   \end{itemize}

\end{itemize}

%Next, we discuss the operations on an NB-tree.% can be implemented to preserve and utilized all the properties and requirements of an NB-tree discussed above.

\if 0
\begin{itemize}
   \item \emph{Cross-s-Node Linkage Property:}
       Let $\mathcal{N}$ be a list of leaf s-nodes in $T_s$ in a traversal order from the left hand side to the right hand side, say
       $N_1, N_2, ..., N_x$.
       If $i < 1_{max}$ (i.e., the s-node (which corresponds to $T_d$) is at the non-leaf level of the structural tree),
       we have the following.
       \begin{itemize}
         \item There is at least one s-key stored in one of the leaf s-nodes in $\mathcal{N}$.
         \item Each leaf s-node in $\mathcal{N}$ contains zero or more s-keys.
         \item Let $K_{min}$ be the smallest s-key in $\mathcal{N}$
         and $K_{max}$ be the largest s-key in $\mathcal{N}$.
            \begin{itemize}
                \item Let $N_{i_{min}}$ be the s-node in $\mathcal{N}$ containing $K_{min}$ where $i_{min} \in [1, x]$.
                   \begin{itemize}
                   \item
                     For each node $N_j$ where $j < i_{min}$ and $N_j$ is in the form of $(P_1, K_1, P_2, K_2, P_3, K_3, P_4, ..., K_{f-1}, P_f, P_{sibling})$,
                        $P_f$ stores the pointer to the root d-node of the data tree $T_d'$ which corresponds to an s-node of the structural tree at level $i+1$
                        such that all keys in $D(T_d')$ are at most $K_{min}$.
                     \item In the d-node $N_{i_{min}}$ in the form of $(P_1, K_1, P_2, K_2, P_3, K_3, P_4, ..., K_{f-1}, P_f, P_{sibling})$,
                         if $K_{min}$ is stored in $K_a$ where $a \in [1, f-1]$, then $P_a$ also stores the pointer to the same root d-node described above.
                     \end{itemize}
                \item Let $N_{i_{max}}$ be the s-node in $\mathcal{N}$ containing $K_{min}$ where $i_{max} \in [1, x]$.
                    \begin{itemize}
                    \item
                        For each node $N_j$ where $j > i_{max}$ and $N_j$ is in the form of $(P_1, K_1, P_2, K_2, P_3, K_3, P_4, ..., K_{f-1}, P_f, P_{sibling})$,
                        $P_f$ stores the pointer to the root d-node of the data tree $T_d'$ which corresponds to an s-node of the structural tree at level $i+1$
                        such that all keys in $D(T_d')$ are greater than $K_{max}$.
                    \item  In the d-node $N_{i_{max}}$ in the form of $(P_1, K_1, P_2, K_2, P_3, K_3, P_4, ..., K_{f-1}, P_f, P_{sibling})$,
                         if $K_{max}$ is stored in $K_b$ where $b \in [1, f-1]$, then $P_{b+1}$ also stores the pointer to the same root d-node described above.
                    \end{itemize}
            \end{itemize}
          \item For each s-key $K_{current}$ in $\mathcal{N}$ where $K_{min} < K_{current}$ and $K_{current} < K_{max}$,
               \begin{itemize}
                  \item ...
               \end{itemize}
       \end{itemize}
\end{itemize}

\hrulefill

More formally, consider a B-tree $T$ with fanout $f$, i.e., each node has at most $f$ children. Let $T_i$ be the collection of nodes in the $i$-th level of the tree, with $T_0$ including only the root. We keep $T_0$ in the main memory, while the rest of the tree will be an on-disk component (they can be cached in main memory if there is more space). Assume that we impose an order on the nodes of $T$ at each level of the tree depending on the smallest key in each node, and let $T_i^j$ be the $j$-th node of the $i$-th level of $T$. For a traditional B-tree, $T_i^j$ is a list of elements including between $\frac{f-1}{2}$ to $f-1$ number of elements.

However, we define $T_i^j$ as a B$^+$-tree of size $s$ (size refers to the number of elements) with branching factor $B$. We will refer to the nodes of the B-tree as \textit{s-nodes} (for structural node) and the B-tree itself will be referred to as the \textit{structural tree}. Each s-node is a B$^+$-tree and the nodes of an s-node will be referred to as \textit{r-nodes} (for regular nodes).

Each s-node, which is a B$^+$-tree, will include two types of elements, \emph{r-elements} (regular elements) and \emph{s-elements} (structural elements), which need to satisfy the following requirements. Each s-node (except the leaf s-nodes) can have between $\frac{f-1}{2}$ to $f-1$ number of s-elements (the lower limit does not apply to the roots) and can have any number of r-elements as long as its size (total number of s-elements and r-elements) does not exceed an integer $s$, the maximum size of each s-node. For a leaf s-node, all of its elements are r-elements and it can have $\frac{s}{2}$ to $s$ number of elements. Furthermore, typical B$^+$-tree requirement on node size applies to r-nodes. We will refer to these requirements on the size of the s-nodes and the r-nodes \textit{size requirements}.

Beside the size requirements, an NB-tree needs to make sure that the s-nodes form a B-tree with branching factor $f$. This will be referred to as \textit{structural requirements} and are described bellow.

As mentioned, $T_i^j$ is B$^+$-tree, i.e., the elements at the leaf level of $T_i^j$ have pointers to their actual records, but with two exceptions. First, each s-key, $e_s$, in addition to a pointer to its record, has a pointer to an s-node in the next level (i.e., to a B$^+$-tree $T_{i+1}^k$ for some $k$) of the structural tree. Secondly, each r-node at the leaf level, in addition to a pointer to its siblings, keeps a pointer to an s-node in the next level of the structural tree (i.e., to a B$^+$-tree $T_{i+1}^k$ for some $k$) These extra pointers are used to enforce a B-tree structure on the s-nodes and how they are created will be explained later. They will be used in queries to traverse down the structural tree and can be seen as the edges of a B-tree.

Namely, in an s-node $T_i^j$ with $k$ s-elements $e_s^i$ sorted in ascending order, for an s-key $e_s^i$, the NB-tree rooted at the s-node pointed to by $e_s^i$ only contains the elements that are less than $e_s^i$ but larger than or equal to $e_s^{i-1}$. This requirement will be referred to as \textit{structural requirement}. This property means that when querying for a key, we will only need to query one of the at most $f$ children of the s-node for the key, resulting in the reduction of the search space by a logarithmic factor which provides the main advantage of NB-trees over LSM-trees that do not posses such a mechanism.

Next we will move on to describing how each operation on an NB-tree is performed.
\fi

%New items to be inserted in $T$ are first inserted in the root s-nodes and are then move along the path to the leaf s-node they should be inserted in. They move down along the path to the leaf whenever the s-node becomes full. When the s-node becomes full, only the r-elements are flushed down to its children. After the r-elements reach the leaf s-node, they become s-elements. s-elements and s-nodes follow a normal B-tree procedure to be inserted in $T$, and a node splits when it has more number of s-elements than allowed, as described in more details bellow.

\subsection{Insertions}\label{sec:design:insertion}
In an NB-tree, we keep the root s-node as an in-memory component and any insertion into the tree is first performed on the root s-node. In this section, we will first provide the overall algorithm for insertion and prove its correctness. Then, we provide more details on the algorithm implementation and show its time complexity in Section \ref{sec:merge}.

\subsubsection{Algorithm.}\label{sec:NBTreeDesign:insertion:algo} An insertion of a key-value pair $K$ and $V$ into an NB-tree $T$ works as follows. $K$ is always first inserted as an r-key into the root s-node, in which one of the following three cases will occur. (1) Insertion of an r-key into a leaf s-node, (2) insertion of an s-key into a non-leaf s-node or (3) insertion of an r-key into a non-leaf s-node.

Before we give the details of these 3 cases, we present two important points.
The first point is the initialization step of the insertion algorithm.
Initially, the NB-tree contains only one s-node (which corresponds to an empty data tree). Obviously, this s-node is a root s-node but it is also a leaf s-node.
When we do an insertion for the first few key-value pairs as r-keys, we execute the operation under Case (1) (i.e., Insertion of an r-key into a leaf s-node).

The second point is the situation in which we execute the operation under Case (2) or Case (3).
Specifically, when we do the insertion operation for the first point, 
the root s-node in the structural tree may become oversize. If the root s-node is a non-leaf s-node, we will insert the r-keys in the root s-node to its children (which corresponds to Case (3)).  Moreover, some times we split some of the s-nodes into two and insert their median key into their parent s-node and change the role of the key (if it is an r-key) from an r-key to an s-key (which corresponds to Case (2)).



\textit{Case 1. Insertion of an r-key into a leaf s-node.} In this case, the insertion of an r-key $K$ into the s-node is identical to a B$^+$-tree insertion. After the insertion, we check whether the s-node is oversize, i.e., it contains more than $s$ keys. If that happens, we perform a \textit{split operation} (discussed bellow below in more details). we split the s-node into two, recursively insert the smaller half of the keys into one and the larger half into another and recursively insert the median of the key, $K_m$, as an s-key (corresponding to Case (2)) into the parent of the split s-node (creating a new s-node as their parent if such an s-node doesn't exist). Note that the median key, $K_m$ is moved up one level in the structural tree, and that $K_m$ has now become an s-key.

\begin{example}
Figure~\insFigNo(a) shows the insertion process under Case (1).
Specifically, we insert 1, 2, 8, 9, 15, 16, 20, 21 and 32 into the NB-tree. 
\end{example}

\textit{Case 2. Insertion of an s-key into a non-leaf s-node.} The insertion of an s-key, $K$, in an s-node, $T_i^j$, only happens when one of the children of $T_i^j$ has been split and $K$ is the median key that has been moved up. Thus, an s-key is always and only inserted into a non-leaf s-node. Let $T_{i+1}^{j_1}$ and $T_{i+1}^{j_2}$ be the two s-nodes whose split has resulted in inserting $K$ in $T_i^j$, where keys of $T_{i+1}^{j_1}$ are less than $K$ and keys of $T_{i+1}^{j_2}$ are larger or equal. The insertion of an s-key in an s-node is similar to a B$^+$-tree insertion but with minor differences. We initially follow the same procedure as inserting a key into a B$^+$-tree, but with the following two additional steps.

First, $K$ will keep a pointer to the s-node $T_{i+1}^{j_1}$ (more specifically to the root d-node of $T_{i+1}^{j_1}$). Secondly, Let $K_l$ be the smallest s-key in $T_{i}^{j}$ larger than $K$ (or $\infty$ if there are no such keys). Similarly, let $K_s$ be the value of the largest s-key in $T_{i}^{j}$ smaller than $K$ (or $-\infty$ if there are no such keys). Then, all the leaf d-nodes whose largest key is larger than $K_s$ but smaller than $K$ will change their pointer $P_{s-node}$ to point to $T_{i+1}^{j_1}$. Furthermore, all the d-nodes whose largest key is larger than or equal to $K$ but smaller than $K_l$ will change their pointer $P_{s-node}$ to point to $T_{i+1}^{j_1}$.

After the insertion, we will check whether $T_{i}^{j}$ has more than $f-1$ s-keys or not. If it does, we split the s-node in two as follows (the split operation). Consider the median of all the $f-1$ s-keys in the s-node, $K_m$. We recursively insert all the r-keys and s-keys smaller than $K_m$ into one s-node (corresponding to Case (2) or (3)) and all the r-keys and s-keys larger or equal to $K_m$ into another (corresponding to Case (2) or (3)). During the split, if a key is currently an r-key, it will be inserted as an r-key and if it's an s-key it will be inserted as an s-key. Then, we recursively insert $K_m$ into the parent of $T_{i}^{j}$ as an s-key (corresponding to Case (2)). Note that after a split, the two newly created s-nodes will have at least $\lfloor\frac{f-1}{2}\rfloor$ s-keys, but the number of r-keys in each s-node can vary.



\textit{Case 3. Insertion of an r-key into a non-leaf s-node.} In this case, the insertion of an r-key $K$ into the s-node, $T_i^j$, is similar to a B$^+$-tree insertion, but with the following additional steps. First, we perform the B$^+$-tree insertion. Note that a B$^+$-tree insertion can lead to a split of some d-nodes inside the s-node. If such a split does happen, consider the original leaf d-node $N_d$ that is split into $N_s$ and $N_l$, where the former contains the smaller half of the keys in $N_d$. Note that because $T_i^j$ is a non-leaf s-node, all its leaf d-nodes contain a pointer, $P_{s-node}$ to the s-nodes in lower levels (because of the procedure discuss in Case 2 above). Thus, $N_d$ contains a pointer to an s-node. Now, we need to set such a pointer for both $N_s$ and $N_l$. We let the pointer $P_{s-node}$ for $N_l$ be the same as that of $N_d$. For $N_s$, we check whether $N_l$ contains an s-key or not. If it does, we copy the pointer of the smallest s-key in $N_l$ as the $P_{s-node}$ for $N_s$. If it doesn't we use the same pointer as that of $N_l$.

After the insertion, we check whether the total number of keys in $T_i^j$ is more than $s$ or not. If it is, we flush down all the r-keys inside $T_i^j$ to its children as follows (we keep the s-keys intact), in an operation called a \textit{merge}. Suppose that there are $n$ s-keys $K_1$ to $K_n$  in $T_i^j$, sorted in ascending order. Then, in merging down the s-node, all the r-keys that are less than $K_1$ are recursively inserted into the s-node pointed to by $K_1$ (corresponding to Case (1) or (3)), and in general if an r-key is more than or equal to $K_{i-1}$ but less than $K_i$, it will be inserted into the s-node pointed to by $K_i$ (corresponding to Case (1) or (3)). For keys larger than or equal to $K_n$, they will be inserted into child pointed to by $P_{s-node}$ of the last d-node in $T_i^j$. All the r-keys are recursively inserted as r-keys into the children. After the merge, only the $n$ s-keys will remain in $T_i^j$. Note that since $T_i^j$ is not a leaf s-node, its leaf d-nodes each have a pointer to an s-node in the next level of the s-tree, and since the r-keys are removed from the s-node, the leaf d-nodes now contain different keys and their pointers in the $P_{s-node}$ pointer slot need to be updated. The process of setting the leaf d-node pointers can be seen as reinserting the s-keys into the s-node as discussed in Case 2 (we will later how this can be done efficiently in implementation).

\begin{example}
Figure~\insFigNo(a) Figure~\insFigNo(h) show an NB-tree grows based on the insertion algorithm discusses above. Note that an insertion of one element may result in multiple recursive calls, as the algorithm discussed is a recursive algorithm. 
\if 0 to  shows the insertion process under Case (2) and Case (3)
Specifically, we insert 33 into the NB-tree as shown in Figure~\insFigNo(a). Figure~\insFigNo(c) shows the NB-tree after we insert 7 keys, namely 10, 29, 49, 59, 83, 91 and 98.
Figure~\insFigNo(d) shows the NB-tree after we insert key 51. 
Figure~\insFigNo(e) shows the NB-tree after we insert 8 keys, namely 3, 4, 5, 6, 7, 14, 18 and 63.
Figure~\insFigNo(f) shows the NB-tree after we insert key 66. 
Figure~\insFigNo(g) shows the NB-tree after we insert 7 keys, namely 11, 24, 25, 26, 47, 55 and 61.
Figure~\insFigNo(h) shows the NB-tree after we insert key 12. \fi
\end{example}

%Note that how the merge and split operations are implemented is consequential to the performance of NB-trees. We will provide more details on these operations in Section \ref{sec:merge}. But because our merge process involves reading and writing the entire B$^+$-tree of each s-node, we can always ensure that the B$^+$-tree d-nodes are completely full. This will possibly both decrease the height of the tree and also eliminate any wastage of space in the tree.

\begin{theorem}[Insertion Correctness]\label{thm:insertionCorrectness}
After an insertion in an NB-tree using the insertion algorithm discussed above, size requirements and structural requirements are satisfied by an NB-tree and the properties are correct, if they were satisfied before the insertion.
\end{theorem}

\textit{Proof Sketch.} Proof by induction on the number of insertion operations.

\hfill\ensuremath{\square} 

%Finally, similar to LSM-trees, updates and deletion in NB-trees are also performed by inserting records containing the information regarding the deletion and the update operations and follow a similar procedure as what describe above (See Section \ref{sec:deletion} for details).



\subsection{Queries}\label{NB:Query}
Queries in an NB-tree are very similar to a B-tree. For a point query, $q$, we start from the root. We first perform the search in the root s-node which is a B$^+$-tree. If $q$ is found in the s-node, we return it. If not, consider the leaf d-node in the B$^+$-tree who was searched but didn't include $q$. If the leaf d-node contains an s-key whose value is larger than $q$, then consider the pointer from the smallest such s-key to the s-node at the next level of the s-tree. If no such s-key exists, the leaf d-node contains a pointer to an s-node of the s-tree who also may contain $q$. Either way, the query is recursively performed on subtree rooted at the child s-node, until the subtree is a leaf s-node. If the subtree is a leaf s-node, we perform the query on the B$^+$-tree of the s-node. If the key is found, we return the key-value pair, if not, the key does not exist (See Fig. \queryFigNo for an example). A similar method can be employed for range queries as well.

%We employ a similar method for range queries as well. For a range query from $l$ to $u$, we start from the root, look for $l$ in the B$^+$-tree, until we reach a leaf d-node in the B$^+$-tree. In the leaf d-node, we find the first key whose value is more than or equal to $l$ and start sequentially reading the sibling of the d-node until we find a key larger than or equal to $u$. If there are any s-keys in the d-nodes we scanned from $l$ to $u$, we do the query recursively on the subtree pointed to by each of the s-keys. If there are no s-keys between $l$ and $u$, we do the query recursively on the s-node pointed to by the first leaf d-node encountered when looking for $l$. if the subtree is a leaf s-node, we perform a range query on the B$^+$-tree at the node and return the result.

\begin{theorem}[Query Performance]\label{thm:queryPerformance}
When a query is performed for a key using the algorithm discussed above, if the key exists in the NB-tree, the algorithm will return the key-value pair in $O(\log_B s \log_f \frac{N}{s})\times(\TSeek+\TSeqR)$, and will return \textit{not found} with the same time complexity otherwise.
\end{theorem}

\textit{Proof Sketch.} The correctness of the query operation follows from the cross-s-node linkage property and the fact that each s-node is a B$^+$-tree. The time complexity follows from the fact that height of each s-node is $O(\log_B s)$ and height of the s-tree is $O(\log_f \frac{N}{s})$.

\hfill\ensuremath{\square} 


\subsection{Deletion and Updates}
In order to perform deletions or update the values of a record, similar to LSM-trees, we insert a new record with the key of the record to be deleted or modified into the structure and mark this new record as a deletion or an update. Because the new record has the same key as the record to be modified, when the new record moves down the tree it will, at some point coexist in the same s-node with the record to be modified. This is because if they are both in the same level of the tree, they both must be in the same s-node, unless there are duplicates of the record with the same key spanning more than one node of the tree (this is because of the cross-s-node linkage property). As a result, we can treat deletions and updates in the same way as insertions and the same analysis applies to these operations as well. Note that if there are duplicates of that key-value spanning more than one node, we need to scan all the nodes containing the duplicates in our query and insertion operations.

\subsection{Parameters}
NB-trees have two parameters, $f$ and $s$. $f$ provides a trade-off between insertion cost and query cost (and consequently insertion time and query time) while $s$ provides a trade-off between the number of seeks performed per insertion and query cost. The value of $s$ typically depends on how expensive seeks are, but typically, to allow for fast insertions, it is set to the order of tens or hundreds of mega bytes. $f$ is typically set to a number on the order of 10 for write intensive workloads, and its increase affects insertion much more than query, as the insertion time linearly depends on $f$ but query time's dependence is only logarithmic. Section \ref{exp:NBTree} provides an empirical analysis for possible values of $f$ and $s$.


\if 0

\begin{algorithm}[tb]
	\caption{Performing Inserts: $I(T, T_s, K, r_or_s)$} \label{algo:insert}
	\begin{algorithmic} [1]
		\REQUIRE An NB-tree $T$, a subtree $T_s$ of $T$ into which a key $K$ is to be inserted and a boolean $r_or_s$ showing whether $K$ is an s-key or an r-key.
		\STATE Let $R$ be the root s-node of $T_s$
		\STATE Let $l$ be the leaf d-node of $R$ that $K$ should be inserted in
		\IF {$K$ is an s-key}
			\STATE Insert $K$ in $l$ using a B$^+$-tree insertion procedure
			\IF {$R$ is not a leaf s-node}
				\STATE \parbox[t]{\dimexpr\linewidth-\algorithmicindent}{Let $p_s$ be a pointer to a child s-node of $R$ with the maximum largest key that is smaller than $K$ \strut}
				\STATE \parbox[t]{\dimexpr\linewidth-\algorithmicindent}{Let $p_l$ be a pointer to a child s-node of $R$ with the minimum smallest key that is larger or equal to$K$\strut}
				\STATE Add the pointer $p_s$ to $K$
				\STATE \parbox[t]{\dimexpr\linewidth-\algorithmicindent}{From $l$, move to the leaf d-nodes whose values are smaller than $K$ and add the pointer $p_s$ to the end of the d-nodes until reaching an s-key or the first leaf node.\strut}
				\STATE \parbox[t]{\dimexpr\linewidth-\algorithmicindent}{From $l$ and including $l$, move to the leaf d-nodes whose values are larger than or equal to $K$ and add the pointer $p_l$ to the end of the d-nodes until reaching an s-key or the last d-node\strut}
			\ENDIF
		\ELSE
			\STATE Insert $K$ in $l$ using a B$^+$-tree insertion procedure
			\IF {$R$ is not a leaf s-node and $l$ was split during the B$^+$-tree insertion}
				\STATE let $l_1$ contain the smaller half of $l$ and $l_2$ the larger half
				\STATE Let $p_2$ be the pointer $P_{s-node}$ existing at the end of $l$.
				\STATE \parbox[t]{\dimexpr\linewidth-\algorithmicindent}{Let $p_1$ be the pointer of the smallest s-key of $l_2$ to $R$'s child. If $l_2$ has no s-keys, let $p_1$ be the same as $p_2$.\strut}
				\STATE Add $p_1$ to the end of $l_1$ and $p_2$ to the end of $l_2$.
			\ENDIF	
		\ENDIF	
		\IF {$size(R) \leq s$ and number of s-keys in $R$ is at most $f-1$}
			\STATE \textbf{return}
		\ENDIF	
		\IF {$R$ is a leaf node or number of s-keys in $R$ is more than $f-1$}
			\STATE Let $P$ be the parent of $R$ in the $T$
			\STATE Let $m$ be the median of keys in $R$
			\STATE \parbox[t]{\dimexpr\linewidth-\algorithmicindent}{Create two nodes $R_1$ and $R_2$ and insert all the keys less than $m$ in $R_1$ and more than $m$ in $R_2$. Let $P$ be the parent of both $R_1$ and $R_2$\strut}
			\STATE Insert $m$ in $P$ as an s-key.
			\STATE \textbf{return}			
		\ENDIF
		\FOR {each s-key $K$ in $R$}
			\STATE \parbox[t]{\dimexpr\linewidth-\algorithmicindent}{Insert all existing r-keys less than $K$ into the child of $R$ pointed to by $K$.\strut}
			\STATE Remove all such keys from $R$.
		\ENDFOR
		\STATE \parbox[t]{\dimexpr\linewidth-\algorithmicindent}{Insert remaining r-keys to the remaining child of $R$. Remove all such keys from $R$.\strut}
%		\STATE \textbf{return}			
	\end{algorithmic}
\end{algorithm}


\begin{algorithm}[tb]
	\caption{Performing Queries: $Q(T, q)$} \label{algo:queries}
	\begin{algorithmic} [1]
		\REQUIRE An NB-tree $T$ and a value $q$
		\ENSURE The key $q$ stored in the data structure
		\STATE Let $R$ be the root of $T$
		\STATE Search $R$ for $q$. Let $l$ be the leaf of $R$ that should contain $q$
		\IF {$l$ contains $q$}
		\STATE \textbf{return} $q$ from $l$
		\ENDIF
		\IF {$R$ is a leaf node}
		\STATE \textbf{return} Not Found
		\ENDIF
		\IF {$l$ contains an s-key larger than $q$}
		\STATE Let $p$ be the smallest s-key larger than $q$ in $l$
		\STATE Let $T'$ be the subtree $p$ points to
		\STATE \textbf{return} $Q(T', q)$
		\ELSE
		\STATE Let $T'$ be the subtree the leaf $l$ points to
		\STATE \textbf{return} $Q(T', q)$
		\ENDIF
	\end{algorithmic}
\end{algorithm}

\fi



\input{example.tex}

\if 0
\subsection{Example}
\subsubsection{NB-tree}
Figure \insFigNo shows an NB-tree for which the size of an s-node is set to be 4 pages (each pages can fit up to 4 keys in this example) and the branching factor is set to be 3. The root of the NB-tree is always kept in memory while the rest of the tree is kept in memory. The keys with a black background in the figure are the s-key that are inserted in the s-tree structure while the key in white background are r-keys in the d-node. Note that leaves have no s-keys, so all the inserted keys in the leaves are shown in white background. For instance, in Fig. \insFigNo (a), all the keys are in white background because they are all inserted in a leaf of the tree, while in Fig. \insFigNo (c), the white keys in the root of the tree are in a white background because they are r-keys in the root, except for 15 which is an s-key in the root.

In Fig. \insFigNo (a), keys are inserted into the in-memory component of the tree, which has initially only one node. But when 33 is inserted into the tree in Fig \insFigNo (b), the node becomes full, it splits into two and its median is pushed to the node in the upper level. Then, in Fig. \insFigNo (c), new keys are inserted into the root node of the tree. When the root becomes full again (Fig. \insFigNo (d)), only the r-keys (not the s-keys in a black background) are flushed down to the leaves. The same process happen in Fig \insFigNo (e) and \insFigNo (f), but this time the leaf s-nodes has to split (because it will contain more than 4 pages otherwise) and write its median, which is 49, in the root.

Fig \insFigNo (g) again shows new keys being inserted in the root. When the root becomes full, the r-keys will be flushed down to the leaf nodes. However, the leaf nodes become full and will have to split. Splitting of the leaf nodes will cause the median of each of the split nodes to be written the root. However, because the fanout of the tree is 3, all the non-leaf s-nodes can have at most 3-1=2 s-keys. Thus, the root will have to split as well, the result of which is shown in Fig \insFigNo (h).

Fig \queryFigNo shows the situation after more keys are inserted into the tree, after the root has overflown and the r-keys are flushed down to the next level. When the query for key 20 is performed, the pages in the highlighted are of the tree will be read, by following the pointers from the root.

Note that in the NB-tree, the leaf d-nodes of the B$^+$-tree in the s-nodes will have pointers to the s-nodes in the next level of the NB-tree to speed up the query time. Furthermore, each s-key will also have a pointer to an s-node in the next levels.


\fi

==> Old/parameters.tex <==
\if 0 \section{Setting the Parameters}\label{sec:NB:param}
An NB-tree has two parameters, size of each node, $s$ and fanout of each node $f$. The root of the tree has to fit in the node which means that $s$ cannot be larger than the memory size. We can set the parameters based on our workload. If the proportion of insertions operations and query operations to the total operations in the workload are $\lambda$ and $1-\lambda$, then we can aim at optimizing the total time taken for the operations. Note that it is always possible to set the parameters empirically, as discussed in Section \ref{sec:exp}.

If we know the workload parameter $\lambda$, we can write an objective function in terms of $\lambda$ based on the analysis in Section \ref{sec:NBTreeDesign} and \ref{sec:merge}. Note that, firstly, differentiating such a formulation and solving for zero will not have a closed-form solution, and thus, we will need to use numerical methods to solve the problem. Secondly, the expression to be minimized is an upper bound on the actual time, and the actual time for the workload is instance dependent (depending on the distribution of the operations for instance). Therefore, the result of optimization will not necessarily give us the optimal value we hoped for, but, it may provide a good estimate for what the parameters should be, as the values will minimize the upper bound. We omit the details on optimization here for the sake of space. 
\fi
\if 0, based on the worst case analysis provided in Section \ref{sec:NBTreeDesign}.

\begin{equation*}
\begin{split}
O(&\lambda\log_f(\frac{N}{s})\times\big[(\frac{s}{s-f}\times\frac{f}{B})\TSeqW + (\frac{1}{s-f}\TSeek)\big] + \\ 
&(1-\lambda)\log_B s \log_f \frac{N}{s}\times(\TSeek+\TSeqR))
\end{split}
\end{equation*}
\fi
%However, if we are more only concerned with the insertion performance, we can optimize the above expression only for insertions by setting $\lambda = 0$. Although this optimization is also only minimizing the upper bound, but it will have a closed-form solution which can be useful in setting the parameters.

\if 0
\subsection{Insertion Intensive Workload}
Based on the insertion cost discussed above, the larger the value of $s$ (for a constant $f$), the smaller the insertion time will be. However, because the root of the tree will have to be memory resident, $s$ has to be smaller than the maximum possible memory space allocated to the tree. In real-world systems, to minimize insertion time, we will set its value to be as large as possible long as $s$ elements can fit in memory.

On the other hand, the larger the value of $f$, the smaller the height of the tree will be, but each merge will take more time. Thus, the effect of $f$ on insertion time is not clear. However, regarding query cost, the larger the value of $f$ is, the smaller the time of the query will be, because the height of the tree becomes smaller.

Because we are dealing with a write-intensive workload, we aim at finding the value of $f$ for which the insertion time is minimum. Because the insertion time in an NB-tree is dependent on the data inserted into the tree (even the order of insertion of the elements affects the time), no value of $f$ will minimize the insertion time for all the instances. As such, here we will provide a value of $f$ that minimizes the upper bound on the insertion time. For this, we need to minimize the function $c(f) = O(\log_f(\frac{N}{s})\times\big[(\frac{s}{s-f}\times\frac{f}{B})\TSeqW + (\frac{1}{s-f}\TSeek)\big])$. Same as above, we assume that $f$ is at most a constant fraction of $s$. This will imply that, $\frac{1}{s-f} = O(\frac{1}{s})$. Therefore, we can rewrite $c(f)$ as $O(\log_f(\frac{N}{s})\times\big[(\frac{f}{B})\TSeqW + (\frac{1}{s}\TSeek)\big])$. Note that in the function, only $f$ is a variable. We can treat $s$ as a constant because for any value of $f$, $c(f)$ monotonically decreases as $s$ increases. $N$ is a constant for a dataset of a specific size and $\TSeqW$, $\TSeek$ and $B$ depend on the machine the data structure is running on. The minimization task becomes a standard calculus optimization problem. The theorem below shows for what value of $f$, the upper bound on insertion time is minimum.

\begin{theorem}
	The maximum insertion time $c(f) = O(\log_f(\frac{N}{s})\times\big[(\frac{f}{B})\TSeqW + (\frac{1}{s}\TSeek)\big])$ has  its minimum value when $f$ is equal to $e\times W(e^{\frac{B\times \TSeek}{e\times s\times \TSeqW}})$, where $W(x)$ is the Lambert W function and $e$ is Euler's number.
\end{theorem}

\textit{Proof}. First note that we can write $\log_f(\frac{N}{s})$ as $\frac{\ln\frac{N}{s})}{\ln f}$ where $\ln$ is the natural logarithm function. Then, differentiating $c(f)$ with respect to $f$ gives us
$$
c'(f) = \ln\frac{N}{s}(\frac{\TSeqW}{B}\times(\frac{\ln f -1}{(\ln f)^2}) - \frac{\TSeek}{s}\times \frac{1}{f(\ln f)^2})
$$
setting $c'(f)$ equal to zero we need to solve the equation 

\begin{equation}\label{eq:minf:1df}
\frac{\TSeqW}{B}\times f\ln f - \frac{\TSeqW}{B}\times f - \frac{\TSeek}{s}=0
\end{equation}


which implies 

$$
\frac{f}{e}e^{\frac{f}{e}} = e^{\frac{B\times \TSeek}{e\times s\times \TSeqW}}
$$

Thus, using the product logarithm function (also known as Lambert W function), we can write $f$ as

$$
f = e\times W(e^{\frac{B\times \TSeek}{e\times s\times \TSeqW}})
$$

To ensure that this value of $f$ corresponds to a minimum value, we need to calculate $c''(f)$ which is equal to  

$$
c''(f) = \ln\frac{N}{s}(\frac{\TSeqW}{B}\times(\frac{2\ln f -(\ln f)^2}{f(\ln f)^4}) + \frac{\TSeek}{s}\times (\frac{2\ln f +(\ln f)^2}{f^2(\ln f)^4}))
$$

Since $f$ and $\frac{N}{s}$ are greater than 1, then $c''(f)$ is greater than zero if and only if 

\begin{equation}\label{eq:minf:2df}
\frac{\TSeqW}{B}\times(f + f - f\ln f) + \frac{\TSeek}{s}\times (2 + \ln f) > 0
\end{equation}

By substituting $f-f\ln f=-\frac{\TSeek\times B}{\TSeqW\times s}$ from equation \ref{eq:minf:1df} into \ref{eq:minf:2df} (which holds at the point where $c'(f) = 0$) we will get

$$
\frac{\TSeqW}{B}\times f - \frac{\TSeek}{s} + \frac{\TSeek}{s}\times (2 + \ln f) > 0
$$

Which means

\begin{equation}\label{eq:minf:2df2}
\frac{\TSeqW}{B}\times f + \frac{\TSeek}{s} + \frac{\TSeek}{s}\times (\ln f) > 0
\end{equation}

Since $f$ is greater than 1 and all other parameters are non-negative, equation \ref{eq:minf:2df2} will always hold true which in turn implies that $c''(f)$ will be greater than zero at the point where $c'(f)$ is zero, i.e. $f = e\times W(e^{\frac{B\times \TSeek}{e\times s\times \TSeqW}})$ corresponds to a minimum value for the function $c(f)$.

\hfill\ensuremath{\square}


\fi

==> Old/proofs.tex <==
\section{Proofs}
\textit{Proof of Theorem \ref{thm:insertionCorrectness}.} Assume that an NB-tree satisfies the requirements before an insertion. We show that the requirements will be satisfied after the insertion as well. Firstly, the size and structural requirements will be satisfied after the insertion, as the size of the s-nodes affected and the number of s-keys are checked and split or merge operations are performed to ensure the sizes are valid. Secondly, we need to show that the cross-s-node linkage property is also satisfied after an insertion. Note that after a key is inserted into the root, it only moves between nodes through merge or split operations. Thus, we need to show that the merge and split operations do not cause the violation of this property. The merge operation, when it is flushing down a key, inserts the key in a child that is pointed to by the smallest s-key larger than the key (or the last child otherwise), which means it will result in a tree that satisfies the structural requirement. Furthermore, the fact that when an s-node is split the median s-key is inserted into its parent and the keys are split into two s-nodes based on whether they are smaller than the median or not also shows the correctness of the split operation.% (the NB-tree split operation is similar to B-tree split operation, and it's correctness follows the B-tree operation's correctness).

\hfill\ensuremath{\square} 

\textit{Proof of Theorem \ref{thm:queryPerformance}.} \textit{Correctness.} The correctness of the query procedure follows from the B-tree structure of NB-tree. Consider the point query $q$ performed on the NB-tree $T$. The query is initially performed on the root of $T$, the B$^+$-tree $T_0^0$. The query includes a traversal from the root d-node of $T_0^0$ to a leaf d-node $N_d$ that could include $q$. If $N_d$ includes $q$, we are done. If $N_d$ doesn't include $q$, and $T_0^0$ is a leaf d-node (This means that $T$ only contains one leaf s-node which is a normal B$^+$-tree) it implies that $T$ doesn't include $q$ and hence the query is done as well. 

If $T_0^0$ is not a leaf node, consider the case that $N_d$ includes an s-key that is larger than $q$. Let $K_1$ to $K_n$ be the sorted list of s-keys in $T_0^0$ with $K_1$ being the smallest, for some integer $n$. Let $T_K$ be the subtree rooted at the node pointed to by the pointer of an s-key $K$. Let $K_i$ be the smallest s-key in $N_d$ that is larger than $q$. Note that based on the cross-s-node linkage property, the subtree $T_{K_i}$ includes keys that are larger than $K_{i-1}$ but less than or equal to $K_i$, and no other disjoint subtree includes any key whose value is between $K_{i-1}$ and $K_i$ (assume $K_0$ is $-\infty$). Thus, we only need to recursively search $T_{K_i}$. If $N_d$ does not include an s-key larger than $q$, $N_d$ has pointer $P_{s-node}$ that satisfies the same properties because of the cross-s-node linkage property and the same argument follows. This shows the query will return the key if it exists. %Correctness of range queries follows from a similar argument.


%Second, the case that $N_d$ does not include an s-key larger than $q$. Again, let $K_i$ be the smallest s-key whose value is larger than $q$. $K_i$ will also be the smallest s-key whose value is larger than the maximum value in $N_d$, because $N_d$ doesn't include an s-key larger than $q$. Then, $N_d$ itself will have a pointer to the subtree $T_{K_i}$. Same as before, $T_{K_i}$  is the only subtree that includes keys larger than $K_{i-1}$ and less or equal to $K_i$. Thus, we only need to recursively search $T_{K_i}$. %TODO: last child?


\textit{Time Complexity}
%TODO: Floating Tree? change the depth according to the number of items in the buffer?
%TODO: Multiple nested levels?
Assume that the NB-tree has $N$ keys. The s-tree, has fanout $f$ and each of the d-trees have fanout $B'$ which is at least $B$. Assume that each d-node is written on a separate disk page. Note that each s-node is at most of size $s$, which means searching each s-node has cost $O(\log_B s)$. Furthermore, the height of the s-tree is $O(\log_f \frac{N}{s})$. Therefore, the cost of querying the data structure is $O(\log_B s \log_f \frac{N}{s})$ which can be written as $O(\log_f s \log_B \frac{N}{s})$.

Note that each page read for a query includes a seek, so the query time will be $O(\log_B s \log_f \frac{N}{s})\times(\TSeek+\TSeqR)$.

\hfill\ensuremath{\square} 



\textit{Proof of Theorem \ref{thm:timeInsertion}.} We assume that we posses at least three disk heads, using which we can read from two disk locations and write in another location simultaneously %without needing the disk head to move between locations and thus incurring no seeks during the reading of two locations and writing to the other (%for more discussion on how this is possible and our methodology when it isn't possible 
(see Section \ref{sec:opt:discHead} for more discussion). This assumption means that we can sequentially scan the d-nodes of $C_i^1$ up to $C_i^k$ with one of the disk heads, and scan d-nodes of $P_i$ sequentially at the same time, while using the other disk head to write sequentially the output of the M\&S operation.

In the worst-case, all the keys have to pass through all the levels of the s-tree which means there will be at most $\frac{N}{s-f}$ s-node overflows (size of s-nodes becoming larger than $s$) at each level (because number of r-keys flushed down is at least $s-f$). For each s-node that has overflowed, we need to read the s-node and all its siblings, together with the children of the s-node. Thus, we have total of $O(\frac{s}{B}(f))$ page accesses for each overflow. The height of the tree is $O(\log_f(\frac{N}{s}))$ because the leaf s-nodes of the NB-tree will have at least $\frac{s}{2}$ keys and each non-leaf s-node at least $\frac{f}{2}$ keys (except the root). Therefore, we have a total of $O(\frac{N}{s-f}\times\frac{s}{B}(f)\times\log_f(\frac{N}{s}))$ I/Os for s-node overflows. Thus, the total cost amortized over $N$ insertions is $O(\frac{s}{s-f}\times\frac{f}{B}\times\log_f(\frac{N}{s}))$. 

For each overflow, a constant number of pages I/Os include seeks and the rest are sequential (we need to keep track of the location of the first leaf d-node in each s-node. We can do this by keeping this information in memory, as it is small, or by storing the location in the root d-node of the s-node which is pointed to by the s-node in the previous level. Otherwise, we will have to perform $O(\log_B s)$ seeks). This is possible because of the sibling sequentiality property and the number of disk heads available. For handling each overflow taken is $O(\frac{s}{B}(f)\TSeqW + \TSeek)$. Hence, the amortized insertion time is  $O(\log_f(\frac{N}{s})\times\big[(\frac{s}{s-f}\times\frac{f}{B})\TSeqW + (\frac{1}{s-f}\TSeek)\big])$. 

$f\leq \frac{s}{2}$, so $\frac{1}{s-f} = O(\frac{1}{s})$ and $\frac{s}{s-f} = O(1)$. Therefore, we can write the amortized insertion time as $O(\log_f(\frac{N}{s})\times (\frac{f}{B}\TSeqW + \frac{1}{s}\TSeek))$. Finally, for each overflow, we need to ensure that the adjacent levels are on different hard disks. If this is not the case, we can move one of the levels to another hard disk, which incurs another $O(\frac{s}{B}(f))$ page accesses.%, which does not impact our analysis. Alternatively, using buffering or better planning regarding which disk each level should be written on to avoid such a scenario can help avoid this extra cost (possibly at the expense of more seeks). We do not discuss these details here for the sake of space.
\hfill\ensuremath{\square}

\if 0
\textit{Proof of Theorem \ref{thm:rateGuarantee}.} A BM\&S operation takes at most $O(\log_{f}\frac{N}{s}(\frac{fs}{B}\TSeqW + \TSeek))$ seconds. This has to be less than the time it takes for the main memory s-node to become full, which is $\frac{s-f}{r}$ and the theorem follows.
\hfill\ensuremath{\square}
\fi
